Edit Distance in Near-Linear Time: it's a Constant Factor

We present an algorithm for approximating the edit distance between two strings of length $n$ in time $n^{1+\varepsilon}$ up to a constant factor, for any $\varepsilon>0$. Our result completes a research direction set forth in the recent breakthrough paper [Chakraborty-Das-Goldenberg-Kouck\`y-Saks, FOCS'18], which showed the first constant-factor approximation algorithm with a (strongly) sub-quadratic running time. The recent results of [Kouck\`y-Saks, STOC'20] and [Brakensiek-Rubinstein, STOC'20] have shown near-linear time algorithms that obtain an additive approximation, near-linear in $n$ (equivalently, constant-factor approximation when the edit distance value is close to $n$). In contrast, our algorithm obtains a constant-factor approximation in near-linear time for any input strings. In contrast to prior algorithms, which are mostly recursing over smaller substrings, our algorithm gradually smoothes out the local contribution to the edit distance over progressively larger substrings. To accomplish this, we iteratively construct a distance oracle data structure for the metric of edit distance on all substrings of input strings, of length $n^{i\varepsilon}$ for $i=0,1,\ldots,1/\varepsilon$. The distance oracle approximates the edit distance over these substrings in a certain average sense, just enough to estimate the overall edit distance.

==> cad.tex <==
\section{Proof of Theorem~\ref{thm:cadGuarantees}}
\label{sec:cad}

\subsection{Algorithm (Alex old)}
\label{sec:CADalgo}

\ns{I was thinking that $\theta$ should be a-priori fixed for all intervals (additive error) and we iterate over different values of $\theta$ in the main subroutine rather than for each pair of intervals. I believe it may help with triangle inequality?}


Suppose the input strings are $I_1$ and $I_2$. We iterate over target
costs $c\in E_w$ and for which we compute the following $q_c(I_1,I_2)$
as well as the symmetric $q_c(I_2, I_1)$ for given intervals $I_1, I_2
\in \IC_{m}$. We construct an alignment graph $H$, similar to the edit
distance dynamic programming, and run shortest path on it. Denoting $\theta =
c/w$ and $\lambda = m/w'$, we construct the directed graph $H$ as follows.

The vertices are $V_{p,q}$ where $p \in w'\cdot [0,\lambda]$ and $q\in p+\theta w'\cdot [0,\lambda]$. For each node
$V_{p,q}$, we add the following edges to $H$:
\begin{itemize}
	\item $V_{p,q} \to V_{p + w',q + w'}$ of cost $\distG_{w'}(I_1 + p,I_2 + q)$ (diagonal edges).
	\item $V_{p,q} \rightarrow V_{p,q\pm \theta w'}$ of cost
          $\theta w'$ (gap edges).
\end{itemize}

Now we run the shortest path from vertex $(0,0)$ to $(w,w)$. This
gives us $q_c(I_1,I_2)$. The final distance is
$$\cad(I_1,I_2)=\min_{c\in E_w} q_c(I_1,I_2)+q_c(I_2,I_1)+c.$$

It is immediate to note that the runtime is $O(|E_w|\cdot \lambda^2)$
since, for each fixed $c$ we have $O(\lambda^2)$ nodes and there are
$O(1)$ edges coming out of each node.

\subsection{Analysis: bounds on $\cad$}

\begin{lemma}
$\cad_w(X_i,Y_j)\ge \ed(X_i,Y_j)$.
\end{lemma}

\begin{proof}
Suppose the $\cad$ minimum is achieved for some $c$ and
$q_c(I_1,I_2)$.

Any path in the graph $H$ induces an $\ed$-alignment between strings
$X_i$ and $Y_j$. In particular, a diagonal edge of cost
$\distG_{w'}(I_1 + p,I_2 + q)$ matches substring $X_{i+p,w'}$ and
substring $Y_{j+q,w'}$ with cost $\distG(i+p,j+q)\ge
\ed(X_{i+p},Y_{j+p})$. Using gap edges corresponds to
deleting/inserting positions into the string $Y_j$.
\end{proof}

We now note that $\cad(I_1,I_2)$ is within $O(1)$-factor of the
shortest path in the graph $H$ where we have all gap edges $V_{p,q}
\rightarrow V_{p,q\pm 1}$.

\begin{lemma}
$    \min_{\pi\in \Pi}\sum_{i\in
      [n]}\tfrac{1}{w}\cad_w(X_{i,w},Y_{\pi(i),w})\le O(C)\cdot \ed(x,y).
$
\end{lemma}
\begin{proof}
Consider the alignment $\pi$ that minimizes the cost $k_\pi=\sum_{i\in
  [n]} \tfrac{1}{w'}\distG_{w'}(X_{i,w'},Y_{\pi(i),w'})\le C\cdot
\ed(x,y)$. For convenience, define $\pi(n+i)\triangleq n+i$ for $i\ge
1$. Now, for fixed $d\in [w]$, we have that,
$$
\sum_{i=0}^{n/w'-\lambda} \left|\pi((i+1)w'+d)-\pi(iw'+d)-w'\right|\le
O(1)\cdot|\pi^{-1}(\bot)|\le O(k_\pi).
$$

      
Now consider $s_d=\sum_{i=0}^{n/w-1}
\cad_w(X_{iw+d,w},Y_{\pi(iw+d),w})$. We have that, 
$$
s_d
\le \sum_{i=0}^{n/w'-1} O(1)\cdot
(\distG(X_{iw'+d,w'},Y_{\pi(iw'+d),w'})+
\left|\pi((i+1)w'+d)-\pi(iw'+d)-w'\right|)
$$
$$
\le \sum_{i=0}^{n/w'-1} O(1)\cdot
\distG(X_{iw'+d,w'},Y_{\pi(iw'+d),w'})+
O(k_\pi).
$$

Hence
$$
\sum_{i\in
  [n]}\tfrac{1}{w}\cad_w(X_{i,w},Y_{\pi(i),w})
=\tfrac{1}{w}\sum_{d\in[w]} s_d\le \tfrac{1}{w}\lambda\sum_{i=0}^{n}
\distG(X_{i,w'},Y_{\pi(i),w'})+O(k_\pi)=O(C)\cdot \ed(x,y).
$$

Hence the claim follows.
\end{proof}

\subsection{Analysis: $\cad$ is a metric}

Identity follows the fact that $\distG$ is a metric, and for $c=0$, we
get $q_0(I,I)=0$. Symmetry follows from the definition of $\cad$.

It remains to prove the triangle inquality. Consider three intervals
$I_1, I_2, I_3$; we want to prove that:
$$
\cad(I_1,I_3)\le \cad(I_1,I_2)+\cad(I_2,I_3).
$$

There exist constants $c_{12},c_{23}\in E_w$ such that
$\cad(I_1,I_2)=q_{c_{12}}(I_1,I_2)+q_{c_{12}}(I_2,I_1)+c_{12}$, and
also $\cad(I_2,I_3)=q_{c_{23}}(I_2,I_3)+q_{c_{23}}(I_3,I_2)+c_{23}$.

Fix $c\in E_w$. 




  


  
  






 

 












 





	



==> complexity.tex <==
\subsection{Complexity Analysis}


\begin{lemma}\label{lm::delete_dense}
	In each ``While'' iteration we identify and remove from $\RC_x$, $\tilde{\Omega}(1)$ fraction of dense nodes at step \ref{alg::dense_delete}. 
\end{lemma}

We define (recursively) the variable
$$ \widehat{\psi_{j,\SC}^\chi}(q_x) = \max\left\{\psi_{j,\SC}^\chi(q_x),\sum_{q' \text{ a child of } q_x} \tfrac{|q' \cap \SC|}{|q_x \cap \SC|} \cdot \widehat{\psi_{j,\SC}^\chi}(q')\right\}$$

For leaves, this means $\widehat{\psi_{j,\SC}^\chi}(v) = \psi_{j,\SC}^\chi(v)$ by convention.

We also define $\widehat{\psi_{j,\SC}}(q_x) = \sum_\chi \widehat{\psi_{j,\SC}^\chi}(q_x)$ and $\widehat{\psi_{j}}(q_x) = \min\{ \widehat{\psi_{j,\XC}}(q_x),\widehat{\psi_{j,\RC_x}}(q_x)\}$.
	We show the following claims.


		
		\begin{claim}\label{cl::node_phi_psi}
			At the end of each iteration, we have with high probability for any $j \in [m]$,
			\begin{enumerate}
				\item $\sum_{\chi} \phi_{j}^\chi(T_\XC) \geq \tfrac{k\cdot n}{2}$.
				\item For any sub-tree $q_x$, $\widehat{\psi_{j,\RC_x}}(q_x) \leq 2k$.
			\end{enumerate}
		\end{claim}
		
\ns{(2) may not hold?}

to show this claim we first show there exists some cost where a bunch of ``good things'' happen.
\begin{claim}
	Fix cost $c$ and coloring $j$ in some step $t$. There exists some cost $c^* \in E_w \cap O(2^{1/\epsilon^2})$ where %
	$\E_{X \sim \RC_x} \left[\E_{A \sim \RC_x}[\phi_{j,\RC_x}^A(X)]\right] \geq \tfrac{0.9}{\lambda^t}$.
\end{claim}

\begin{proof}
	Fix $X \in \RC_x$. First, we need an anchor sampled $A \in \NC_{c^*}^{\RC_x}(X)$. Assuming such anchor was sampled, we assign $\phi_{j,\RC_x}^A(X) = \tfrac{|\RC_x|}{d_X \cdot \lambda^t}$, where $d_X \approx \max \{\NC_{c^*}^{\RC_x}(X), \NC_{c^*}^{\RC_x}(A)/\beta\}$.
\end{proof}

	\begin{claim}\label{claim::bound_psi}
		Fix $q_x \in T_\XC$ and $\SC \in \{\XC, \RC_x\}$, we have $\widehat{\psi_{j,\SC}}(q_x) = \sum_\chi \min \{ \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\} - h \cdot O(\tfrac{k}{\log n})$%
	\end{claim}
	
	
	
	\begin{proof}
		We prove by induction on tree height $h=h(q_x)$. For leaves, $Q(v)$ contains any matching color, hence the claim follows.
		Assume by induction the claim holds for $h-1$. We partition the colors for 3 group:
		\begin{enumerate}
			\item Colors $\chi$ with $\tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|} \geq \tfrac{1}{\beta \log n}$.
			\item Colors $\chi$ with $\tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|} < \tfrac{1}{\beta \log n}$ and for all $q'$ child of $q_x$, $\widehat{\psi_{j,\SC}^\chi}(q') < 1$.
			\item Colors $\chi$ with $\tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|} < \tfrac{1}{\beta \log n}$ and there exists a child $q'$ with $q_x$, $\widehat{\psi_{j,\SC}^\chi}(q') = 1$.
		\end{enumerate}
		
		For (1), we have $\psi_{j,\SC}^\chi(q_x) = \min\{\tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\}$.%
		
		
				
				For (3), we use Claim \ref{cl::node_phi_psi} to obtain there are at most $2 k \beta$ such colors for $\SC=\RC_x$ (for $\SC=\XC$ there are no such colors possible).

		
		Overall, we have (denoting $\nu_1, \nu_2$ and $\nu_3$ the color sets of (1), (2) and (3) respectively):
		
		\begin{align*}
			\widehat{\psi_{j,\SC}}(q_x) &= \sum_\chi \widehat{\psi_{j,\SC}^\chi}(q_x) \\
				&\geq \sum_{q' \text{ a child of } q_x} \tfrac{|q' \cap \SC|}{|q_x \cap \SC|} \cdot \widehat{\psi_{j,\SC}}(q') + \sum_{\chi \in \nu_1 \cup \nu_3} \widehat{\psi_{j,\SC}^\chi}(q_x) - \sum_{\chi \in \nu_1 \cup \nu_3} \sum_{q' \text{ a child of } q_x} \tfrac{|q' \cap \SC|}{|q_x \cap \SC|} \cdot \widehat{\psi_{j,\SC}}(q') \\
				&\geq \sum_{\chi \in \nu_2} \sum_{q' \text{ a child of } q_x} \tfrac{\rho_{\SC}(q')|q'|}{\rho_{\SC}(q_x)|q_x|}\cdot \tfrac{\phi_j^\chi(q')}{\rho_{\SC}(q')|q'|} - (h-1 )\cdot O(\tfrac{k}{\log n})  + \sum_{\chi \in \nu_1} \psi_{j,\SC}^\chi(q_x) \\
				&=   \sum_{\chi \in \nu_2} \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|} - (h-1 )\cdot O(\tfrac{k}{\log n}) + \sum_{\chi \in \nu_1}\min\{\tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\} \\
				&\geq \sum_\chi \min \{ \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\} - (h-1) \cdot O(\tfrac{k}{\log n}) - \sum_{\chi \in \nu_3} \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|} \\
				&\geq \sum_\chi \min \{ \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\} - (h-1) \cdot O(\tfrac{k}{\log n}) -  \tfrac{2k\beta}{\beta \log n} \\
				&\geq \sum_\chi \min \{ \tfrac{\phi_j^\chi(q_x)}{\rho_{\SC}(q_x)|q_x|},1\} - h \cdot O(\tfrac{k}{\log n})
		\end{align*}
				
				
		as needed.
		
		\ns{okay, I think this one is done.}
		

		
		
		
		
		
		
		
		\end{proof}


		
				\begin{lemma}\label{lm::prob_dense}
			Fix subtree $q_x$ of height $h=h(q_x)$ and $\epsilon \in [0,1]$. 			$$\Pr_{v \in q_x \cap \RC_x} [v \text{ in a dense sub-tree}] \geq \tfrac{\sum_j \widehat{\psi_j}(q_x)}{5\cdot m \cdot k} - \tfrac{\epsilon^2 \cdot h}{50}$$
		\end{lemma}
		\begin{proof}
			We prove by induction on $h$. Leaves are defined as dense  $\psi_{j}(q_x) \geq \tfrac{\epsilon^2}{100} \cdot k$, hence for non-dense leaves the claim follows. For dense leaves we use Claim \ref{cl::node_phi_psi} to show probability is at most 1. 
			
			Now we assume the claim holds for $h-1$ ,and show for sub-trees of height $h$. We consider the following cases.
			
			\paragraph{Dense Sub-tree.} If for $\tfrac{\epsilon^2}{100}$ partitions we have $\psi_{j}(q_x) \geq \tfrac{\epsilon^2}{100} \cdot k$, then $q_x$ is a dense sub-tree and the claim follows.
			
			\paragraph{Sparse Sub-tree.} Otherwise, we have $\sum_j \psi_j(q_x) \leq \tfrac{\epsilon^2}{50}\cdot m \cdot k$, and since $\widehat{\psi_{j}}(q_x) \leq \psi_{j}(q_x) + \sum_{q' \text{ a child of } q_x} \tfrac{|q' \cap \RC_x|}{|q_x \cap \RC_x|} \cdot \widehat{\psi_{j}}(q')$, we obtain,
			
			\begin{align*}
				\Pr_{v \in q_x \cap \RC_x} [v \text{ in a dense sub-tree}] &= \sum_{q' \text{ a child of } q_x} \frac{|q' \cap \RC_x|}{|q_x \cap \RC_x|} \cdot \Pr_{v \in q' \cap \RC_x} [v \text{ in a dense sub-tree}] \\
				&\geq \sum_{q' \text{ a child of } q_x} \frac{|q' \cap \RC_x|}{|q_x \cap \RC_x|} \cdot \left(\frac{\sum_j \widehat{\psi_j}(q')}{5\cdot m \cdot k} - \frac{\epsilon^2 \cdot (h-1)}{50}\right) \\
				&\geq \left(\sum_{q' \text{ a child of } q_x} \frac{|q' \cap \RC_x|}{|q_x \cap \RC_x|} \cdot \frac{\sum_j \widehat{\psi_j}(q')}{5\cdot m \cdot k}\right) - \frac{\epsilon^2 \cdot (h-1)}{50} \\
				&\geq \left(\sum_{j \in [m]} \sum_{q' \text{ a child of } q_x} \frac{|q' \cap \RC_x|}{|q_x \cap \RC_x|} \cdot \frac{\widehat{\psi_j}(q')}{5\cdot m \cdot k}\right) - \frac{\epsilon^2 \cdot (h-1)}{50} \\
				&\geq \left(\sum_{j \in [m]} \frac{\widehat{\psi_j}(q_x) - \psi_j(q_x)}{5\cdot m \cdot k}\right) - \frac{\epsilon^2 \cdot (h-1)}{50} \\
				&\geq \left(\frac{(\sum_{j}\widehat{\psi_j}(q_x)) - \tfrac{\epsilon^2}{50}\cdot m \cdot k}{5\cdot m \cdot k}\right) - \frac{\epsilon^2 \cdot (h-1)}{50} \\
				&\geq \left(\sum_{j \in [m]} \frac{\widehat{\psi_j}(q_x)}{5\cdot m \cdot k}\right) - \frac{\epsilon^2}{50} - \frac{\epsilon^2 \cdot (h-1)}{50} \\
				&= \left(\sum_{j \in [m]} \frac{\widehat{\psi_j}(q_x)}{5\cdot m \cdot k}\right) - \frac{\epsilon^2 \cdot h}{50}
			\end{align*}
			
			as needed.
			
		\end{proof}

	
\begin{proof}[Proof of Lemma \ref{lm::delete_dense}]
From Lemma \ref{lm::prob_dense}, we have,
$$\Pr_{v \in \RC_x} [v \text{ in a dense sub-tree}] \geq \tfrac{\sum_j \widehat{\psi_j}(T_\XC)}{5\cdot m \cdot k} - \tfrac{\epsilon^2 \cdot \epsilon^{-2}}{50}$$

Which is lower bounded from Lemma by
$$\Pr_{v \in \RC_x} [v \text{ in a dense sub-tree}] \geq \tfrac{\sum_{j}\sum_{\chi}\phi_j^\chi(T_\XC)/n - O_\eps(m \cdot k /\log n)}{5\cdot m \cdot k} - \tfrac{1}{50} \geq \tfrac{m\cdot k \cdot n / 2n - O_\eps(m \cdot k /\log n)}{5\cdot m \cdot k} - \tfrac{1}{50} \geq 0.08 - O_\eps(1/\log n)$$
\end{proof}


\begin{lemma}\label{lm::partition_size}
	Fix $t \in [\log_\lambda n]$. Each color $\chi$ in each coloring
        $\kappa_j^{t+1}$ is assigned to at most $ n \cdot \tO_\eps(m^{t} \cdot
k^{t} \cdot \log^{O(t)}(n) \cdot \beta^{2t} \cdot \lambda^{-t})$
        intervals (ie, that's the max size of a part in partition).
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lm::partition_size}]



First, we claim whp, $| \PC_{\kappa_j^t}^\chi \cap \XC| = \tilde{\Theta}(n\cdot \lambda^{-t})$ (ie, each color $\chi \in [\lambda^t]$ is assigned to %
$\tilde{\Omega}(n\cdot \lambda^{-t})$ $x$-axis intervals) in each step and we analyze for $y$-axis.

 \ns{this should be easy to prove I think, similar to the previous Lemma based on scoring, but if not easy we can simply combine colors, for example by combining small size colors with large size, to ensure no color is too small on the $x$ side.}
 


  For $y$, we make an inductive assumption $| \PC_{\kappa_j^t}^\chi \cap \HC| \leq \tO_\eps(m^{t-1} \cdot
k^{t-1} \cdot \log^{O(t - 1)}(n) \cdot \beta^{2t-2} \cdot n \cdot \lambda^{1-t})$ for step $t-1$ (in step 1 we have $2n$) and show for step $t$.
  
  
For each anchor $A$ sampled in each partition $j \in [m]$, we have,
 $$\sum_{v
  \text{ leaf in } T_y} \phi_j^A(v) \leq \beta\cdot
\tfrac{n}{\lambda^t} \cdot \tfrac{| \PC_{\kappa_j^t}(A) \cap \HC|}{|
  \PC_{\kappa_j^t}(A)\cap \WC|}$$
\aanote{where does the $\beta$ factor come from?}
\aanote{where does the $\tfrac{| \PC_{\kappa_j^t}(A) \cap \HC|}{|
  \PC_{\kappa_j^t}(A)\cap \WC|}$ ratio come from?
  \textsc{ClusterAnchor} seems to minimize $d_{c^*+c}/d_{c^*}$, which
  may be very different ($d$ includes counts for both $x$ and $y$)}

   (since we choose the minimum fraction in \textsc{ClusterAnchor}). We use the $x$-axis argument and induction hypothesis and this quantity becomes, 
  $\sum_{v
  \text{ leaf in } T_y} \phi_j^A(v) \leq \beta\cdot
\tfrac{n}{\lambda^t} \cdot \tO_\eps(m^{t-1} \cdot
k^{t-1} \cdot \log^{O(t - 1)}(n) \cdot \beta^{2t-2} \cdot n \cdot \lambda^{1-t}) \cdot \tilde{\Theta}(n^{-1}\cdot \lambda^{t-1})= n\cdot \tO_\eps(m^{t-1} \cdot
k^{t-1} \cdot \log^{O(t-1)}(n) \cdot \beta^{2t-1}\cdot \lambda^{-t})$, hence the total potential of $A$ in $T_y$ is bounded by the above.   For each node $q_y$ we color $\chi_{A,j}$, we requires $\Omega(|q_y|/\beta)$ potential on one hand, and we color $O(|q_y|)$ intervals on the other hand. Therefore, $\chi_{A,j}$ is added to the color set of $n\cdot \tO_\eps(m^{t-1} \cdot
k^{t-1} \cdot \log^{O(t-1)}(n) \cdot \beta^{2t}\cdot \lambda^{-t})$ intervals for each anchor $A$ sampled in partition $j$.
  

  
  

  We also note by Lemma~\ref{lm::delete_dense} that in each step we iterate $\tO(1)$ times, and in each time, we sample $k$ anchors in each of $m$ partitions for each color. Hence the total number of anchors per color is $\tO(m \cdot k)$, %
  and hence each color will contain $n\cdot O_\eps(m^{t} \cdot
k^{t} \cdot \log^{O(t)}(n) \cdot \beta^{2t} \cdot \lambda^{-t})$ intervals as needed.




\end{proof}

\begin{corollary}[Complexity]\label{lm::main_complexity}
	\textsc{MatchIntervals}($\WC, \HC, \GC_w, c$) takes $T(n) = O_\eps(n^{1 + O(\eps)} \cdot \log^{O(1/\eps)} n \cdot T_{\cad})$ time.
\end{corollary}
\begin{proof}
	At each step $t$, we sample $m \cdot k \cdot \lambda^t$ anchors and compare each one to matching partitions and repeat until $\RC_x = \emptyset$. From Lemma \ref{lm::delete_dense}, we have $\tO(1)$ such rounds, and from Lemma \ref{lm::partition_size}, each time we compare each anchor to $n \cdot \tO_\eps\left( \tfrac{m \cdot k \cdot \beta^{2}}{\lambda}\right)^t$ intervals. Therefore, we invoke a total of $m \cdot k \cdot \lambda^t \cdot n \cdot \tO_\eps\left( \tfrac{m \cdot k \cdot \beta^{2}}{\lambda}\right)^t = m \cdot k \cdot n \cdot \tO_\eps\left( m \cdot k \cdot \beta^{2}\right)^{1/\epsilon}$ $\cad$ queries (since $t \leq 1/\epsilon)$. Which simplifies to $ n \cdot O_\eps\left(n^{2\eps^2/\epsilon} \cdot \log^{O(1/\eps)} (n)\right) = O_\eps\left(n^{1+2\eps} \cdot \log^{O(1/\eps)} (n)\right)$ $\cad$ queries. %
	
Therefore, the matching complexity is $T(n) = O_\eps(n^{1 + O(\eps)} \cdot \log^{O(1/\eps)} n \cdot T_{\cad})$.

\end{proof}


==> correctness-prelims.tex <==
\subsection{Correctness analysis preliminaries}
\label{sec:analysisPrelims}

Before continuing with the correctness analysis, we establish some
auxiliary statements. 

\input{notation-new.tex}

\vspace{2mm}
\paragraph{Distortion Resilient Distance Properties.}
We show some properties of Distortion Resilient Distance from Def. \ref{def::dd}. Recall that $\dd_F(p,q) = \sum_{i:p_i > F\cdot q_i} |p_i|$. First, we show multiplication by scalars.

\begin{fact}\label{ft::dd_scalar}
	Fix $p,q \in \R^n_+$ and scalars $a, b \in \R_+$. We have
		$\dd_F(a\cdot p,b\cdot q) = a\cdot \dd_{F\cdot \tfrac{b}{a}}(p,q)$
\end{fact}
\begin{proof}


		$$\dd_F(a\cdot p,b\cdot q) = \sum_{i:\tfrac{a p_i}{b q_i} > F} |a p_i| = a \sum_{i:\tfrac{p_i}{q_i} > \tfrac{bF}{a}} |p_i| = a\cdot \dd_{F\cdot \tfrac{b}{a}}(p,q)$$
\end{proof}




We also show a bound on the $\ell_1$ normalization of vectors.

\begin{fact}\label{ft::dd_norm}
	Fix $p,q \in \R^n_+$. We have,
	$$\dd_{2 \cdot F^2}\left(\tfrac{p}{\normo{p}},\tfrac{q}{\normo{q}}\right) + \dd_{2 \cdot F^2}\left(\tfrac{q}{\normo{q}},\tfrac{p}{\normo{p}}\right) \leq 4\cdot \left(\tfrac{\dd_{F}(p,q)}{\normo{p}} + \tfrac{\dd_{F}(q,p)}{\normo{q}}\right)$$
\end{fact}

\begin{proof}
	By fact \ref{ft::dd_scalar}, we have that,
	$$\dd_{2 \cdot F^2}\left(\tfrac{p}{\normo{p}},\tfrac{q}{\normo{q}}\right) + \dd_{2 \cdot F^2}\left(\tfrac{q}{\normo{q}},\tfrac{p}{\normo{p}}\right) = \tfrac{1}{\normo{p}} \cdot \dd_{2 \cdot F^2 \cdot \tfrac{\normo{p}}{\normo{q}}}\left(p,q\right) + \tfrac{1}{\normo{q}} \cdot \dd_{2 \cdot F^2 \cdot \tfrac{\normo{q}}{\normo{p}}}\left(q,p\right)$$
	
	Now, consider a case where $\tfrac{\normo{p}}{\normo{q}} \in
        [1/2F,2F]$, then we have that, using the observation that
        $\dd_F(a,b)$ is decreasing in $F$:
		$$\dd_{2 \cdot F^2}\left(\tfrac{p}{\normo{p}},\tfrac{q}{\normo{q}}\right) + \dd_{2 \cdot F^2}\left(\tfrac{q}{\normo{q}},\tfrac{p}{\normo{p}}\right) \leq \tfrac{1}{\normo{p}} \cdot \dd_{F}\left(p,q\right) + \tfrac{1}{\normo{q}} \cdot \dd_{F}\left(q,p\right)$$
		
	Otherwise, assume w.l.o.g $\tfrac{\normo{p}}{\normo{q}} > 2F$,
        then on one hand we have that $\dd_{F}\left(p,q\right) \geq
        0.5\normo{p}$, and hence the RHS of the claim is at least $4 \cdot 0.5 = 2$. On the other hand, $\dd_{2F^2}\left(\tfrac{p}{\normo{p}},v\right)\leq 1$ for any $v$, and similarly for $q$, and hence the LHS is at most 2 and the claim follows.
	
\end{proof}



	






\vspace{2mm}
\paragraph{Alternative Counting for $\Lambda$ balls.} When bounding certain parameters, we use the following simple combinatorial claim:

\begin{claim}\label{cl::lambda_ball_func}
	Fix coloring $\kappa$, parameter $\zeta \geq 1$ and function $f: \IC \rightarrow \R_+$. Then,
	
	$$
	\sum_{I \in \IC} \mu_\kappa(I,\un) \cdot f(\Lambda_\kappa^\zeta(I)) = \sum_{I \in \IC} \mu_\kappa(\Lambda_\kappa^\zeta(I),\un) \cdot f(I) \leq 2\zeta f(\IC).
	$$
\end{claim}
\begin{proof}
	The proof follows immediate by counting the contribution of each $f(I)$ to elements in $\Lambda_\kappa^\zeta(I)$. Formally:
	
	$$
	\sum_{I \in \IC} \mu_\kappa(I,\un) \cdot f(\Lambda_\kappa^\zeta(I)) = \sum_{I \in \IC} \mu_\kappa(I,\un) \cdot \sum_{J \in \Lambda_\kappa^\zeta(I)} f(J) = \sum_{I \in \IC}  \sum_{J \in \IC} \1[\mu(\text{SEB}(I,J)\footnote{SEB$(I,J)$ = smallest enclosing ball containing both intervals},\un) \leq \zeta] \cdot \mu_\kappa(I,\un) f(J)
	$$
	
	Now, by change of summation, such quantity equals

	$$
	 \sum_{J \in \IC}  \sum_{I \in \IC} \1[\mu(\text{SEB}(I,J),\un) \leq \zeta] \cdot \mu_\kappa(I,\un) f(J) = \sum_{J \in \IC} f(J) \cdot \sum_{I \in \Lambda_\kappa^\zeta(J)} \mu_\kappa(I,\un) = \sum_{J \in \IC} \mu_\kappa(\Lambda_\kappa^\zeta(J),\un) \cdot f(J).
	$$
	
	And since $\mu_\kappa(\Lambda_\kappa^\zeta(J),\un) \leq 2\zeta$, we conclude:
	
		$$
	\sum_{I \in \IC} \mu_\kappa(I,\un) \cdot f(\Lambda_\kappa^\zeta(I)) = \sum_{I \in \IC} \mu_\kappa(\Lambda_\kappa^\zeta(I),\un) \cdot f(I) \leq 2\zeta f(\IC).
	$$
	
	as needed.
	
\end{proof}



==> denseDistance.tex <==
\section{Structural Properties: C-Matchable everywhere}

\subsection{Alignment of intervals}


Let $A$ be the optimal alignment between $x$ and $y$. In
other words, we have
$$
\pi:[n]\to [n]\cup \{\bot\},
$$ satisfying the following:
\begin{itemize}
\item injective and monotone on $\pi^{-1}(\bot)$;
\item $\pi$ is 2-Lipshitz;
\item
  $x[i]=y[\pi(i)]$ for all $\pi(i)\neq \bot$;
\item $|\pi^{-1}(\bot)|=O(\ed(x,y))$.
\end{itemize}

\begin{claim} When $X_i,Y_i$ are intervals of length $w$, we have:
    $\sum_{i\in[n]} \ed(X_{i},Y_{\pi(i)})\le O(\ed(x,y)\cdot w).$
\end{claim}


\subsection{Matchings of Intervals}

\aanote{write for a generic metric between intervals?}

\begin{definition}
For a set of intervals $\RC \subseteq \IC_w$, a {\em matching} $\MC$ is a
one-to-one assignment of each $x$-interval $X \in \RC \cap \WC_w$ with
a unique $y$-interval $Y \in \RC \cap \HC_w$. Note that matching may
not exist when $|\RC\cap \HC|\neq |\RC\cap \WC|$.
\end{definition}

We will also refer to such pairing as ``blocks'', as they define $w
\times w$ squared blocks in the graph. In general, we care to identify
``cheap'' paths in the graph which consists of ``cheap'' matchings. We
now develop such intuition.

\begin{definition}
	A set of intervals $\RC \subseteq \IC$ is called {\em
          $c$-matchable} if there exists a matching of $\MC$ in which
        $\cad_\GC(X,Y) \leq c$ for each pair $(X,Y) \in (\WC_w \cap
        \RC) \times (\HC_w \cap \RC)$ of the matching.
\end{definition}

We now define boxes which are dense everywhere, meaning every ball around such boxes has a large matchable subset.

\begin{definition}
	A pair of intervals $(X,Y)  \in \WC_w \times \HC_w$ is called
        {\em $c$-dense everywhere} (abbreviated ``$c$-d.e.``) if for any $s>0$, there exists $\MC_c \subseteq \BCs(X,Y)$ which is $c$-matchable with $|\MC_c| \geq sw$.
\end{definition}




The next lemma shows that finding $c$-de matchings will incur a
constant-factor approximation only. In the lemma below, one should
think of $e_i$ as the original distance between $X_i$ and $Y_j$

\begin{lemma}
Fix $\gamma\in(0,1)$, and let $Q_\gamma(A)$ for a multi-set be the
$(1-\gamma)$-quantile of $A$ (e.g., $\gamma=0$ corresponds to max). Fix
numbers $e_1,\ldots, e_n\ge 0$. For $i\in
[n]$, define:
$$
\dd_i=\max_{s\in 2^\N\cap[n]} Q_\gamma(\{e_{i+j} \mid j\in[-s,+s]\}).
$$
Then we have that 
$$
  \sum_{i\in [n]} \dd_{i} \le O(\tfrac{1}{\gamma}\cdot \sum_i
  e_i).
  $$
\end{lemma}


\begin{proof}
For level $l\ge 0$, let $S_l=[-2^l,+2^l]$. For each $i$, let $L_i$ be
the $l$ such that $s=2^l$ is the maximizer of the
$\dd_{i}^\gamma$. Note that this means that $\gamma S_l$ indeces
$j\in[-2^l,2^l]$ satisfy $e_{i+j}\ge \dd_{i}^\gamma\ge e_i$. For level
$l$, let $P_l$ be the set of ``passive'' indeces $i$ such that $L_i<
l$ (i.e., it has already seen it's max-achieving level). At the
beginning $P_0=\emptyset$.

For each interval $i$, we assign a (fractional) potential $\phi_i(l)$,
which starts at 0, and increases with level $l$ until it reaches $\ge
5/\gamma$. We will have the following
invariants, which we prove inductively with $l\ge 0$:
\begin{itemize}
\item
  the sum of all potentials $\sum_{i\in[n]}\phi_i(l)$ is exactly equal
  to the size of $P_l$;
\item
  for any $i\in[n]$ with potential $\phi_i(l)$, there are $\phi_i(l)$
  uniquely-associated indeces $j\in P_l$ (of fractions thereof),
  satisfying $e_j<e_i$ with $|j-i|\le 2^l/2$.
\item
  furthermore, $\sum_{i\in P_l} \dd_i\le \sum_{i\in[n]}\phi_i(l)\cdot e_i$;
\end{itemize}

At level $l\ge 0$, consider an index $i$ such that $L_i=l$; i.e.,
$i\not\in P_l$ but $i\in P_{l+1}$. Let
$M_i\subset i+S_l$ be the set of indeces $i+j\in i+S_l$ that are in the
top $\gamma$-fraction of $e_{i+j}$'s and whose
potential $\phi_{i+j}(l)$ is less than $5/\gamma$. We claim that $|M_i|\ge \gamma
|S_l|/2$. Indeed, consider the opposite: there is a set $K\subset
i+S_l$ with $|K|> \gamma/2\cdot |S_l|$, with each potential $\phi_l(k)\ge
5/\gamma$ for $k\in K$,
where each $e_k$ is larger than $1-\gamma$ fraction of $i+S_l$. By
inductive hypothesis, there are $\ge 5/\gamma\cdot |K|\ge 2.5\cdot
|S_l|$ unique indeces within distance $2^l/2$ of the set $i+S_l$,
which is not possible.

So we have $|M_i|\ge \gamma |S_l|/2$. For each $k\in M_i$, we increase
its potential $\phi_k$ by $1/|M_i|\le 2/\gamma\cdot 3/2^l$ for the
next level. Note that the total potential increase due to $i$ is
$\sum_{k\in M_i} 1/|M_i|=1$ --- hence we think of $i$ being split into
pieces, which is uniquely associated to an index in $M_i$. Note also
that for each $k\in M_i$, we have $e_k\ge d_i$, and also that
$|k-i|\le 2^{l'}/2$ for any subsequent level $l'>l$.

Finally observe that the potential of any node never goes above
$5/\gamma+|S_l|\cdot 2/\gamma\cdot 3/2^l\le O(1/\gamma)$ (the second
term comes from how much increment can be done in one level).

Eventually we reach a level where $P_l=[n]$. Hence, we can bound:
$$
\sum_{i\in[n]} \dd_i \le \sum_{i\in [n]} \phi_i(l) e_i\le
O(1/\gamma)\cdot \sum_{i\in[n]} e_i. 
$$
\end{proof}




==> distG.tex <==
\subsection{Proof of Theorem \ref{thm::clustering_restated} using Lemma \ref{lm::matching_guarantee}}

\begin{proof}[Proof of Theorem \ref{thm::clustering_restated} using Lemma \ref{lm::matching_guarantee}]
  Let $G_w=\cup_c c\cdot G_{w,c}$, and let $\mu(\cdot,\cdot)$ be the
  distance in this graph. For the fast data structure $\GC_w$ built on
  $G_w$, inducing distance $ \distG=\distG_w$, we have that $\mu\le
  \distG\le O(\mu)$.

  To prove the first part of the theorem, consider any two intervals
  $I_1, I_2$, and the shortest path $v_1,\ldots v_k$ between them,
  where $v_1=I_1$ and $v_k=I_k$. We have that $(v_i,v_{i+1})$ is an
  edge is some graph $G_{w,c_i}$, and hence the cost
  $\mu(I_1,I_2)=\sum_{i=1}^{k-1} c_i$. By
  Lemma~\ref{lm::matching_guarantee}, we have that $c_i\ge
  \cad_w(v_i,v_{i+1})$. Hence $\distG(I_1,I_2)\ge
  \mu(I_1,I_2)=c_1+\ldots c_{k-1}\ge \cad_w(v_1,v_2)+\ldots
  \cad_w(v_{k-1},v_k)\ge \cad_w(I_1,I_2)$.

  For the second part, we note that $\mu(I_1,I_2)$ is upper bounded by
  $\sum_{c\in E_w} 2c\cdot (I_1,I_2)\not\in G_{c,w}$. Hence:
  $$
  \sum_{i\in [n]} \mu(X_{i,w},Y_{\pi(i),w})
  \le
  \sum_{i\in [n]} \sum_{c\in E_w} 2c\cdot
  \one{(X_{i,w},Y_{\pi(i),w})\not\in G_{c,w}}
  =
  2\sum_{c\in E_w} c\cdot \sum_{i\in [n]} 
  \one{(X_{i,w},Y_{\pi(i),w})\not\in G_{c,w}}.
  $$

  For fixed $c$, we have that, by Lemma~\ref{lm::matching_guarantee}:
  $$
  \sum_{i\in [n]} 
  \one{(X_{i,w},Y_{\pi(i),w})\not\in G_{c,w}}
  \le
  \sum_{i\in [n]} \one{\cad_w(X_{i,w},Y_{\pi(i),w})\le
    O(c\eps^2)}+O(k_{\Omega(c\eps^2)}).
  $$
  We bound two terms separately:
  $$
  \sum_{c\in E_w}\sum_{i\in [n]} c\cdot \one{\cad_w(X_{i,w},Y_{\pi(i),w})\le
    O(c\eps^2)}\le  \sum_{i\in [n]} O(1/\eps^2)\cdot \cad_w(X_{i,w},Y_{\pi(i),w}),
  $$
  $$
  \sum_{c\in E_w} c\cdot
  O(k_{\Omega(c\eps^2)})=O(\tfrac{1}{\eps^2})\cdot \sum_{c\in E_w}
  c\cdot k_c=O(\tfrac{1}{\eps^2})\cdot \sum_{c\in E_w}
  \sum_{i\in[n]}c\cdot
  \one{\cad_w(X_{i,w},Y_{\pi(i),w})>c}\le O(\tfrac{1}{\eps^2})\cdot\sum_{i\in[n]} 2\cad_w(X_{i,w},Y_{\pi(i),w}).
  $$
  Altogether, we obtain
  $$
  \sum_{i\in [n]} \distG_w(X_{i,w},Y_{\pi(i),w})
  \le
  O(1)\cdot \sum_{i\in [n]} \mu(X_{i,w},Y_{\pi(i),w})
  \le
  O(\tfrac{1}{\eps^2})\cdot\sum_{i\in [n]} \cad_w(X_{i,w},Y_{\pi(i),w}).
  $$

  As for the runtime, it follows immediately from the runtime in
  Lemma~\ref{lm::matching_guarantee}.
\end{proof}



==> global.tex <==
\section{Discretizing Global Densities - Alternative}

To solve for different global densities, focusing on small distances, the idea is to incorporate the slope of matches as well. First, we introduce some further notations.

\subsection{Adjusted Definitions}

To solve for small distances we partition balls into $p = 1/\theta$ diagonal elements. For $\Delta \in [p-1]$, we call $\Lambda^\Delta_s(\A) = \BC_{(\Delta+1) s/p} (\A) \setminus \BC_{(\Delta-1) s/p} (\A)$ the {\em diagonal partitioning} of $\BCs(\A)$.


\ns{Make $\Delta \in \Z$ and perturb $y$-axis shifts}


\begin{definition}
	A pair of intervals $(X,Y)  \in \WC_w \times \HC_w$ is called ``$c$-dense everywhere'' (abbreviated ``$c$-d.e.``) if for any $s>0$, there exists $\MC_c \subseteq \BCs(X,Y)$ which is $c$-matchable with $|\MC_c| \geq s \cdot w$, and moreover, for any $(X^*,Y^*)$ in the matching, we have that $\tfrac{\normint{X-X^*}}{\normint{Y-Y^*}} \in 1 \pm 2\theta$
\end{definition}


\subsection{Density Mass}
We also need a way to measure densities across partitions, for that we first define sets of intervals with similar densities. %

For density $d \in [n]$, density $d \in [n]$, cost $c \in [w]$, family of sets $\FC$ over $\IC_w$ we denote $\JC_c^\FC(d) = \{ I \in \IC_w \mid d_c^\FC(I) = d \}$, meaning all intervals with density $d$. For sets of densities $U \subseteq [n]$, we denote $\JC_c^\FC(U) = \cup_{d \in U} \JC_c^\FC(d)$.

In addition, for sets of intervals $T \subseteq S$ we denote $\mu_S(T) = |T| / |S|$, meaning the mass of $T$ in $S$. We also use the shorthand $\mu(\RC) = \mu_{\IC_w}(\RC)$ and $\mu_{c,\FC,\RC}(d) = \mu_{\RC}(\JC_c^\FC(d) \cap \RC)$, meaning the pdf of $\mu_{\RC}(\JC_c^\FC(d) \cap \RC)$.





Clearly, $\mu_{c,\FC,\RC}([n]) = 1$ for any $\RC$. The idea is therefore that for each matchable set $\MC_c$, there exists some magnitude of density with sufficient mass, i.e. some $U \in \left\{ [d,2d) \mid d \in \{ 1,2,4,8,\ldots,n\} \right\}$ for which the following holds,


$$\mu_{c,\FC,\MC_c}(U) \geq \mu_{c,\FC,\IC_w}(U)$$


\subsection{Density Finder}
In order to use the above, we first develop an algorithm for sampling anchors with pre-defined densities. We show the following Lemma.

\begin{lemma}
	Fix $k, m \in \N$ and $\theta \in (0,1)$, and let $\RC$ be an interval set of size $m$, and $\PC_\FC$ partitioning of $\IC_w$. Let $U_0 = [1,1/\theta]$, and $\UC = \{U_0\} \cup \{(2^{i-1},2^{i}]/\theta\}_{i \in [\log_2 \theta m]}$. There exists a randomized algorithm that runs in $\tilde{O}(km)$ time and outputs $\tO(k)$ intervals (anchors), such that for each $U \in \UC$ with $\mu_{c,\FC,\RC}(U) > \theta$, there exists whp at least $k$ intervals in the set with density in $U$.
\end{lemma} 
\begin{proof}
	The algorithm is the following simple one. Sample uniformly $\tO(k/\theta)$ intervals from $\RC$ and compare each one to $\theta$ fraction of the other intervals in its partition. Output $k$ random candidates for each density level found. 
\end{proof}



\subsection{Adjusted Clustering and Partitioning, and Algorithm}

\paragraph{Adjusted algorithm.}
The algorithm would be adjusted as follows. At each step $t$, we would sample $\tO (2^t / \theta)$ anchors, and compare each one to a much smaller partition as above.

Then, we will adjust the radius according to the number of anchor cluster that obtained similar density.

Before presenting the algorithm, we adjust clustering and partitioning to allow the above.

\paragraph{Adjusted Clustering.} We now discretize the clusters according to their density. For each anchor cluster $\A$, we let $\widehat{d_\A}=|\A|$, meaning the density of the anchor cluster, rounded up to the nearest power of 2. Then we add the cluster to $\CC_{t,\widehat{d_\A}}$. We use that to allow larger radius for densities with smaller mass.

\paragraph{Adjusted Partitioning.}
	For a set $\CC_{t,d}$ of anchor clusters with $s = |\CC_{t,d}| \cdot d$, let $\FC_d = \{ \Lambda_s^\Delta(\A) \mid \A \in \CC_{t,d}, \Delta \in [1/\theta] \}$ be the associated family of diagonal partitions of $\CC_{t,d}$ and let $\FC = \cup_d \FC_d$. We refer to $\PC_\FC$ as the {\em interval partitioning} of $\CC_{t}$.
	


\begin{algorithm}[H]
\caption{Matching Phase - Main Algorithm}
\label{alg::match_main}
\begin{algorithmic}
\Function{MatchIntervals}{$\WC_w,\HC_w,\GC,\theta,c$}.
\Comment $\GC$ is clustering of $\IC_{w/\lambda}$
\State $k \gets \tilde{O}(1/\theta)$; $\A_1 \gets \{X_0,Y_0\}; b \gets n/w; \CC_1 \gets \{(\A_1, b)\}$.
\State Init $G_{w,c}$ as an undirected graph with nodes $\IC_w$ and no edges.
\For{ $t \in [\log_2 n]$} 
\State $\CC_{t+1,d} \gets \emptyset$ for all $d \in \{1, 2,4,8,\ldots ,n \}$.
\For{ $r \in [t]$ }
\For{$[2^t \cdot k ]$}%
\State Sample uniformly $A \sim \WC_w$.
\State Let $\PC_\FC$ be the interval partitioning of $\CC_r$.
\State $\A \gets \textsc{ClusterAnchor}(A,P_{2^{r-t}}(\PC_\FC(A)),\GC,2c)$.
\State $\widehat{d_\A} \gets |\A|$, rounded up to the smallest power of 2.
\If{ $\widehat{d_\A} > \theta \cdot n \cdot 2^{-t}$ }
\State Add edges $\{(A,I) \mid I \in \A \}$ to $G_{w,c}$.
\Else
\State $\CC_{t+1,\widehat{d_\A}} \gets \CC_{t+1,\widehat{d_\A}} \cup \{ \A \}$.
\EndIf
\EndFor
\EndFor
\EndFor
\State \Return $G_{w,c}$. %
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsection{Adjusted analysis - complexity}

Similar to previous section, but now we pay $\theta$ fraction, since diagonal partition saves $\theta$ factor.
\ns{write proof.}

\subsection{Adjusted Analysis - correctness}

We adjust the probability of success Lemma as follows.

\begin{lemma}\label{lm::probpart-adj}
	Fix $l,r,b \geq 1$ and $\eta,\theta > 0$. Let $\CC_{r}$ be a set of anchor clusters. Let $\PC_\FC$ be cluster partitioning of $\CC_r$.%
	Fix $(X, Y) \in \HC_w \times \WC_w$ which is $(2c,l,\eta)$-dense in $\FC$.
	Then, there exists $t > r$ such that for a random anchor $A \sim \WC_w$ at step $t$, we have with at least $\tfrac{\eta \cdot l}{5 \cdot b \cdot 2^{t-r}}$ probability that a call for \textsc{ClusterAnchor} will output an anchor cluster $(\A, s, p)$, with the property that $\cup_\Delta \Lambda^\Delta_{s/2}(X,Y) \subseteq \cup_\Delta \Lambda^\Delta_{s}(\A)$. %
	
\end{lemma}

First, let us claim the probability of success for each $\Delta \in [k-1]$ as follows.

\begin{lemma}\label{lm::probdiag}
	Fix $k \in \N$, $s \geq 1/k$ and $\Delta \in [k]$. Let $\FC$ be family of sets over $\IC$. Fix $(X, Y) \in \HC \times \WC$, and let $\MC^\Delta_c \subseteq \BC_s(X,Y)$ be a $2c$-matchable set with the properties of Definition \ref{def::dense-in-R} (for some $l, \epsilon$), such that for each $(X^*,Y^*) \in \MC^\Delta_c \cap \WC \times \MC^\Delta_c \cap \HC$, we have that $\tfrac{\normint{X-X^*}}{\normint{Y-Y^*}} \in 1 \pm 1/k$.  
	
		Then, there exists $i \in 0 \ldots [\log_2 b]$ such that with at least $\tfrac{\epsilon l}{5 \cdot b \cdot 2^{i}}$ probability, a call to\\
		\textsc{ClusterAnchor}$(A,P_{2^{-i}}(\FC(A)),\hat{\alpha},2\hat{\alpha} c)$ with a uniformly random $A \in \WC$ will output an anchor cluster $(\A, s, p)$ where: (1) $\A \cap \MC_c^\Delta \cap \WC \neq \emptyset$ (2) $\A \cap \MC_c^\Delta \cap \WC \neq \emptyset$, and (3) $|\A|\cdot s \cdot 2^i < 2l$.%
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lm::probdiag}]
First, define $Z_A$ as the event an anchor $A \in \NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)$ will be sampled:

$$Z_A = A \in \NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)$$

Next, let $\A_X = P_{2^{-i}}(\NC_{2c}(A) \cap \WC)$,  $\A_Y = P_{2^{-i}}(\NC_{4c}(A) \cap \HC)$. We define $Z_1, Z_2, Z_3$ for conditions (1), (2) and (3) in the Lemma, respectively:

\begin{align*}
Z_1 &= \exists X' \in \A_X \cap \MC_c^\Delta \\
Z_2 &= \exists Y' \in \A_Y \cap \MC_c^\Delta \\ 
Z_3 &= 2^{i} \cdot |\A_X \cup \A_Y|\cdot s \leq 2l 
\end{align*}



Finally, we define the probability of success:

$$\Pr[\text{success}] \geq  \Pr[Z_A] \cdot \Pr[Z_1, Z_2,Z_3 | Z_A] \geq \Pr[Z_A] \cdot (\Pr[Z_1 | Z_A] \cdot \Pr[Z_2 | Z_A] - \Pr[\neg Z_3|Z_A])$$

Where the last part is true since $Z_1|Z_A$ and $Z_2|Z_A$ are either independent or positively correlated. %



Now, by Fact \ref{fact::setdense} $|\NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)| = \tfrac{|\MC_c^*|\cdot d^{\FC}_{2c}(\MC_c^*)}{d^{\MC_c^*}_{2c}(\MC_c^*)} \geq \tfrac{\epsilon l}{2^{i}\cdot b \cdot \theta}$ %
, we have, 
$$\Pr[Z_A] \geq \tfrac{|\NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)|}{b/\theta_c} \geq \tfrac{\epsilon l}{b \cdot 2^{i}}$$


Conditioned on finding such anchor, we have:
$$\Pr[Z_1 | Z_A] = \Pr[Z_2 | Z_A] = 1- (1-2^{-i})^{d^{\MC_c^*}_{2c}(\MC_c^*)} \geq 1- \exp(-2^{i} \cdot 2^{-i}) = 1-e^{-1} > 0.63$$

(noting that since $\MC_c^*$ is a ``matchable'' set, then all neighborhoods contains the same amount of $x$-axis and $y$-axis intervals). 

Finally, since for all $(X^*,Y^*)$ matches in $\MC_c^*$, $d_{4c}^{\FC}(Y^*) \cdot \max\{\normint{X^* - X},\normint{Y^* - Y}\} \leq l$, and we sub-sample with prob. $2^{-i}$, then by the Chernoff bound for $|\FC(A)| = \omega(2^{i})$ we have $\Pr[\neg Z_3|Z_A] = o(1)$. We can conclude the probability of success is 
$$\Pr[\text{success}] \geq \tfrac{(0.63^2 - o(1)) \cdot \epsilon l }{b \cdot 2^{i+1}} > \tfrac{\epsilon \cdot l }{5 \cdot b \cdot 2^{i}}$$

as needed.

\end{proof}

For proving Lemma \ref{lm::probpart-adj}, we aggregate probabilities over all possible $\Delta$ as follows.

\begin{proof}[Proof of Lemma \ref{lm::probpart-adj}]
Let $\MC_{c}^*$ be a $2c$-matchable set with the properties of Definition \ref{def::dense-in-R}. Let $\MC_{c}^\Delta = \MC_c^* \cap \Lambda_{s/2}^\Delta(X,Y)$. Let $\epsilon_\Delta = |\MC_c^\Delta|\cdot d^{\FC}_{2c}(\MC_c^\Delta)\cdot \theta / l$, and note that since $(X,Y)$ is $(2c,l,\epsilon)$-dense in $\FC$ and any pair of the matching is in some $\Lambda_{s/2}^\Delta(X,Y)$, then $\sum_\Delta \epsilon_\Delta \geq \epsilon$.

For $\Delta \in [k-1]$, we invoke Lemma \ref{lm::probdiag}, and obtain there exists some $i_\Delta$ which satisfy the Lemma with $\tfrac{\epsilon_\Delta \cdot l }{5 \cdot b \cdot 2^{i}}$ probability. Now, define $\epsilon_\Delta^i = \epsilon_\Delta \cdot \mathbb{1}[i_\Delta=i]$ and let $\epsilon^i = \sum_\Delta \epsilon^i_\Delta$. Finally, let $i^* = \text{argmax}_i \epsilon^i$. Since there are at most $\log b$ possible values for $i$, then by pigeon hole principle we have that $\epsilon^{i^*} = \tilde{\Omega}(\epsilon)$. Now noticing that the probabilities of success are mostly independent, for $q^* = r+i^*$, we will have with probability $\tilde{\Omega}(\tfrac{\epsilon \cdot l }{b \cdot 2^{q^* - r}})$ that $\MC_c^* \cap \A$ contains both $X^* \in \Lambda^\Delta_{s/2}(X)$ and $Y^* \in \Lambda^\Delta_{s/2}(Y)$ for some $\Delta \in [k-1]$.




The Lemma immediately follows, since $\cup_\Delta \Lambda^\Delta_{s/2}(X,Y) \subseteq \cup_\Delta \Lambda^\Delta_{s}(X^*,Y^*) \subseteq \cup_\Delta \Lambda^\Delta_{s}(\A)$ (where the second step follows the triangle inequality).


\ns{check / prove formally last part.}

\ns{formalize dependencies.}

\ns{perhaps we can do better by say birthday paradox at some regimes?}



\end{proof}



==> match-analysis.tex <==
\subsection{Interval Matching - High Level Concept}

To match $2c$-d.e. boxes, the high level idea is to make $\log n$ iterations, and in each one, we make $\tilde{O}(n)$ $\cad$ approximations using Theorem \ref{thm::cad_approx}, with the goal of ``disqualifying'' constant portion of the $\WC_w \times \HC_w$ graph (with high prob) so after $O(\log n)$ we can match essentially all $2c$-d.e. boxes using $\tilde{O}(n)$ total estimations. %
Our matching algorithm consists of three building blocks: Anchor Sampling, Clustering and Partitioning. The overall matching algorithm will again interleave between each of these steps until convergence.%

\subsection{Clustering Subroutine} To find ``matches'' in the proximity of all $2c$-d.e. boxes, we use the following main subroutine. 



\vspace{2mm}

\textsc{ClusterAnchor}$(A,\RC,\GC, c)$. Fix %
anchor $A \in \IC_{\lambda w}$, clustering $\GC$ and interval set $\RC \subseteq \IC_{\lambda w}$, this subroutine approximates $\cad_{\GC}(A,I)$ for all $I \in \RC$, and returns set $\A$ of all matching $x$ intervals with estimated cost $\leq 2c$ and $y$ intervals with estimated cost $\leq c$ (denoted ``anchor-cluster'').%



\begin{algorithm}[H]
\caption{Matching Phase - Clustering Subroutine}
\begin{algorithmic}
\label{alg::disc.subroutines}	

\Function{ClusterAnchor}{$A,\RC, \GC, c$}
\State Estimate $\cad_\GC(A,I)$ using the estimator of Theorem \ref{thm::cad_approx} for all $I \in \RC$ (denoted $\widehat{c_{A,I}}$).
\State $\A \gets \{ A \} \cup \{ X \in \RC \cap \WC_{\lambda w} \mid \widehat{c_{A,X}} \leq 2c\}\cup \{ Y \in \RC \cap \HC_{\lambda w} \mid \widehat{c_{A,Y}} \leq c\}$

\State \Return $\A$.
\EndFunction

\end{algorithmic}
\end{algorithm}

\subsection{Interval Partitioning}
Before presenting our interval matching algorithm, we define interval partitioning based on sets of anchor clusters as above.
Fix $\FC$ to be a family of interval sets over $\IC$. For $I \in \IC$, define $\PC_\FC(I) = \cup_{\substack{\RC \in \FC \\ I \in 
	\RC}} \RC$.
	To complete notation, we define $\PC_\FC(S) = \cup_{I \in S}\PC_\FC(I)$, $\NC_c^\FC(I) = \NC_c(I) \cap \PC_\FC(I)$, $d_c^{\FC}(I) = |\NC_c(I) \cap \PC_\FC(I)|$, and the corresponding definitions for sets of intervals.
	
	For a set $\CC$ of anchor clusters, let $\FC = \{ \BC_s(\A) \mid (\A,s) \in \CC \}$ be the associated family of balls of $\CC$.
	We refer to $\PC_\FC$ as the {\em interval partitioning} of $\CC$.
	



\subsection{Interval Matching - Main Algorithm} 

To match $2c$-d.e. intervals, our algorithm proceeds as follows. In the below, the operator $P_\delta(S)$ for $\delta \in [0,1]$ is an operator which subsamples $S' \subseteq S$ by keeping each element of $S$ with probability i.i.d $\delta$. Parameter %
$\eta$ (sub-constant) will be fixed later.

\begin{algorithm}[H]
\caption{Matching Phase - Main Algorithm}
\label{alg::discover.int}
\begin{algorithmic}
\Function{MatchIntervals}{$\WC_w,\HC_w,\GC,\theta,c$}.
\Comment $\GC$ is clustering of $\IC_{w/\lambda}$
\State $k \gets \tilde{O}(1/\eta)$; $\A_1 \gets \{X_0,Y_0\}; b \gets n/w; \CC_1 \gets \{(\A_1, b)\}$.
\State Init $G_{w,c}$ as an undirected graph with nodes $\IC_w$ and no edges.
\For{ $t \in [\log_2 n]$} 
\State $\CC_{t+1} \gets \emptyset$.
\For{ $r \in [t]$ }
\For{$[2^t \cdot k ]$}%
\State Sample uniformly $A \sim \WC_w$.
\State Let $\PC_\FC$ be the interval partitioning of $\CC_r$.
\State $\A \gets \textsc{ClusterAnchor}(A,P_{2^{r-t}}(\PC_\FC(A)),\GC,2c)$.
\State $s \gets \tfrac{b}{|\A|\cdot 2^{t+1}}$.
\If{ $s < 1/w$ }
\State Add edges $\{(A,I) \mid I \in \A \}$ to $G_{w,c}$.
\Else
\State $\CC_{t+1} \gets \CC_{t+1} \cup \{ (\A,s) \}$.
\EndIf
\EndFor
\EndFor
\EndFor
\State \Return $G_{w,c}$. %
\EndFunction
\end{algorithmic}
\end{algorithm}


\ns{By keeping only $\tilde{O}(1)$ anchor clusters for each ``band'' of $s$, we should save one $\eta$ factor}


\section{Matching Phase - Analysis}

We now show complexity and correctness of the matching phase. %


\subsection{Matching Analysis - Complexity}
Our task here is bounding the number of $\cad$ estimations of the matching phase, which all occur within the \textsc{ClusterAnchor} subroutine. We note that we have at most $\tilde{O}(1)$ combinations of $(t,r)$, hence it suffices to fix $(t,r)$ and bound the number of $\cad$ estimations of the internal loop.


\begin{claim}%
	Fix $r,t > 0$. For each sampled anchor in the internal loop, we spend $\tilde{O}(n/\eta 2^t)$ $\cad$ estimations.
\end{claim}

\begin{proof}
	We note we have at most $r \cdot 2^r \cdot k$ anchor clusters in $\CC_r$, and for each one $|\BC_{s'}(\A')| \leq \tfrac{n}{2^{r+1}}$ (since $|\A'|\cdot s' = b/2^{r+1} = n/w 2^{r+1}$ and $|\BC_{s'}(\A')| = |\A'|\cdot s' \cdot w$), hence we expect an anchor to be a member of $\tilde{O}(1/\eta)$ balls, and therefore $|\PC_\FC(A)| = \tilde{O}(\tfrac{n}{2^{r} \eta})$ with some probability.
	
	\ns{move statistics to ball size and bound all probabilities in Lemma $\ref{lm::probpart}$...}
	
	For each such anchor, we make one call \textsc{ClusterAnchor}, and with high probability, such call to \textsc{ClusterAnchor} costs $\tilde{O}(2^{r-t} \cdot |\PC_\FC(A)|) = \tilde{O}(\tfrac{n}{2^t \cdot \eta})$ $\cad$ estimations %
\end{proof}
\begin{corollary}
	Each matching phase costs $\tilde{O}(\tfrac{n^{1+2/\gamma}}{\eta^2})$ time.
\end{corollary}
\begin{proof}
	Fix $r,t\geq 1$ as above. We sample $T_A = 2^t \cdot m  = \tilde{O}(\tfrac{2^t}{\eta})$ anchors. For each one we spend $T_\RC = \tilde{O}(\tfrac{n}{2^t \cdot \eta})$, $\cad$ estimation, each taking $T_{\cad}=\tO((\lambda w)^2 / w^2) = \tO(\lambda^2)$ time according to Theorem \ref{thm::cad_approx}.
	
	Hence the total time is $T_A \cdot T_\RC \cdot T_\cad = \tilde{O}(\tfrac{n \cdot \lambda^2}{\eta^2}) = \tilde{O}(\tfrac{n^{1+2/\gamma}}{\eta^2})$ as needed.
\end{proof}
\subsection{Matching Analysis - Correctness}

First, one can observe that for any $w,c$, any $(I_1,I_2)$ edge added to $G_{w,c}$ is of $\cad_\GC$ at most $c$, and by triangle inequality we can correctly upper bound $\cad_\GC$ for any pair of intervals.

\begin{lemma}
	Fix $w,c$ and $I_1,I_2 \in \IC_w$, such that $d_{G_{w,c}}(I_1,I_2) \leq \alpha$. Then, $\cad_\GC(I_1,I_2) \leq \alpha c$.
\end{lemma}
\begin{proof}
	Since the estimator of Theorem \ref{thm::cad_approx} outputs an upper-bound on $\cad_\GC$, then any edge $(I_i, I_j)$ added to $G_{w,c}$ is of cost at most $\cad_\GC(I_i,I_j)\leq c$. The claim follows triangle inequality.
\end{proof}

The more challenging task is showing that almost all $2c$-d.e. $(X,Y)$ boxes will be matched. For this task, the crux is proving that with high probability, for any step $t$, $(X,Y)$ maintain at least one common ball, meaning we generate some anchor cluster $(\A,s)$ for which $X, Y \subset \BC_{s}(\A)$, and moreover, that $\BC_{s/2}(X,Y) \subseteq \BC_{s}(\A)$ for sufficiently large $s$. The delicacy in the analysis stems from capturing different densities of intervals, both in close proximity to $(X,Y)$ ({\em local density}) as well as in the overall matching ball $\BC_{s'}(\A')$ from some previous step ({\em global density}). 

\vspace{2mm}

For {\em global density}, our approach is to bound the number of {\em $\eta$-globally sparse} intervals, and solve only for {\em $\eta$-dense} intervals. We start by defining pairs which are {\em $\eta$-globally dense} in some partitioning $\PC_\FC$. Those are pairs for which we expect to cluster an $x$-axis and $y$-axis match (whp) in their proximity at some future step $t$.

\begin{definition}\label{def::dense-in-R}
	Fix $c,l,w,\eta > 0$ and let $\FC$ be a family of interval sets over $\IC_w$. We call an interval pair $(X,Y) \in \WC_w \times \HC_w$, ``$(c,l,\eta)$-dense in $\PC_\FC$'' %
	if there exists $\MC_c^* \subseteq \IC_w$ such that the following holds:
	
\begin{enumerate}[a)]
	\item $\MC_c^*$ is $c$-matchable.
	\item $\sum_{Y^* \in \MC_c^* \cap \HC_w} d_c^{\FC}(Y^*) \geq \eta l w$.
	\item For all $(X^*,Y^*)$ in the matching, 
	(1) $Y^* \in \PC_\FC(X^*)$, and \\(2) $d_{2c}^{\FC}(X^*) \cdot \max\{\normint{X^* - X},\normint{Y^* - Y}\} \leq l$.
\end{enumerate}
\end{definition}

Let provide some intuition on the above conditions for the set $\MC_c^*$.
 Condition (a) ({\em matching condition}) ensures that if we sample an anchor $A \in \NC_c(\MC_c^* \cap \HC)$, we have by triangle inequality that $Y^* \in \NC_{c}(A), X^* \in \NC_{2c}(A)$. Condition (b) ({\em density condition}) guarantees the set $\MC_c^* \cap \HC_w$ is sufficiently dense so an anchor from the neighborhood above will be sampled (whp) at some future step $t$ (as will be explained later). Finally, by condition (c) ({\em proximity condition}), we have that once we cluster a matching $(X^*,Y^*)$, then $X$ and $Y$ will be contained in the associated ball $\BC_{s/2}(X^*,Y^*)$. 


\begin{lemma}\label{lm:reps}
	Fix $c,w,n,\eta > 0$ and let $\CC_t$ be a set of anchor clusters generated at some step $t$. Let $\PC_\FC$ be cluster partitioning of $\CC_t$. %
	Then, there exists $\WC_\FC^\eta \subseteq \WC_w$ and $\HC_\FC^\eta \subseteq \HC_w$ such that:
	
	\begin{enumerate}
		\item $|\WC_\FC^\eta|,|\HC_\FC^\eta| \leq \eta n$.
	\item For all $(X,Y) \subseteq \WC_w \setminus \WC_\FC^\eta \times \HC_w \setminus \HC_\FC^\eta$ $2c$-d.e. pairs, if there exists $(\A,s) \in \CC_t$ with $\BC_{s/2}(X,Y) \subseteq \BC_{s}(\A)$, then $(X,Y)$ is also $(2c,b/2^{t+2},\eta)$-dense in $\PC_\FC$.%
	\end{enumerate}
	
\end{lemma}

\begin{proof}[Informal]
Intuitively, fix any $X \in \WC_w$ we care about (i.e. where there exists at least one $c$-d.e. box $X,Y$), then any set of $x$-axis intervals which are part of a $c$-matchable set (for any such $Y$ ) in $\BC_s(X)$ would contain most of the intervals in $\BC_s(X)$. Therefore, unless a constant portion of them are $\eta$-sparse (i.e. sparser than $1-\eta$ portion of the intervals) or very dense (say $1/\eta$ more dense then the average, which by Markov can be for at most $\eta$ portion of intervals), the density and proximity conditions should hold. And there should be a way to bound the number of such $x$-axis intervals. 

For making sure $s$ is ``sufficiently large'' for part (1) in the proximity condition, we note that we require neighborhood densities not to ``collapse'' much faster than factor 2 for each step, but this is very reasonable assumption, as we only have double the anchors, so densities should not change by more than that (and in fact, most of the time will reduce at much slower pace...)

\end{proof}
\ns{Alex, I am still having trouble proving this. I think the first part (say for step 1) should go in somewhat similar way of Lemma \ref{lm::not-cde}. The hard case seems to be when all the sparse intervals are adjacent, and by affecting each other, prevent us from finding $\eta$ portion of the intervals (and this is one of the issues of small distances TBD). Also we don't actually need $\BC_{s/2}(X,Y) \in \BC_s(\A)$, a smaller ball would suffice for $\GC_1$ for example, and even if just a large constant portion of $\BC_{s/2}(X,Y)$ intersects with $\BC_s(\A)$ should be enough. The second part should also not be too hard to prove I think but I am still having trouble doing it. This is also the part I think is the least intuitive in the construction, as from initial observation it appears as if we lose from other ``branching'' factors, but in fact all we care about is that the global densities of $x$-axis intervals don't go down by a lot each step, which should be true with good probability. }

We now present the following key Lemma, in which we analyze the probability of success for a random anchor. Consider $2c$-d.e. boxes where $2c$-matchable sets in their proximity are {\em locally dense}, i.e. their neighborhoods overlap a lot. Then the probability to sample an anchor of the overall neighborhood is relatively small. However, once we found such anchor, we are likely to find a match even if we {\em sub-sample} the neighborhood in some future step $t$.%

\begin{lemma}\label{lm::probpart}
	Fix $l,r,b,w \geq 1$ and $\eta > 0$. Let $\CC_{r}$ be a set of anchor clusters. Let $\PC_\FC$ be cluster partitioning of $\CC_r$.%
	Fix $(X, Y) \in \HC_w \times \WC_w$ which is $(2c,l,\eta)$-dense in $\PC_\FC$.
	Then, there exists $t > r$ such that for a random anchor $A \sim \WC_w$ at step $t$, we have with at least $\tfrac{\eta \cdot l}{5 \cdot b \cdot 2^{t-r}}$ probability that a call for \textsc{ClusterAnchor} will output an anchor cluster $(\A, s)$, with the property that $\BC_{s/2}(X,Y) \subseteq \BC_{s}(\A)$.%
	
\end{lemma}
Finally, we use the above Lemma to show that almost all $2c$-d.e. intervals are certified correctly.
\begin{lemma}
	There exists $\WC^\eta \subseteq \WC_w$ and $\HC^\eta \subseteq \HC_w$ with $|\WC^\eta \cup \HC^\eta| = \tilde{O} (\eta n)$ such that with high probability, the matching phase correctly clusters all $2c$-d.e $(X,Y) \in [\WC_w \setminus \WC^\eta] \times [\HC \setminus \HC^\eta]$ boxes.
\end{lemma}

\begin{proof}
	
	We prove by induction on $t$. For step $t-1$, fix $\WC_{t-1}^\eta \subseteq \WC_w$ and denote $\WC_{t-1} = \WC \setminus \WC_{t-1}^\eta$ and similarly for $\HC_{t-1}^\eta$ and $\HC_{t-1}$. We make the following inductive assumptions hold whp:
	\begin{enumerate}
		\item $|\WC_{t-1}^\eta|, |\HC_{t-1}^\eta| \leq \eta n \cdot (t-1)$.
		\item For each $2c$-d.e $(X,Y) \in \WC_{t-1} \times \HC_{t-1}$, there exists $\CC_{r}$ with $r \leq t-1$ such that $(X,Y)$ is $(2c,b/2^{r+2},\eta)$-dense in $\PC_\FC$, where $\PC_\FC$ is the cluster partitioning of $\CC_{r}$, and moreover, that parameter $t'$ in Lemma \ref{lm::probpart} is at least $t$. %
	\end{enumerate}
	
	We prove for step $t$. Fix $2c$-d.e. pair $(X,Y)$ as in (2) above. If $t' > t$ then the statement is immediately true for such pair at step $t$ as well (as $t'$ is therefore at least $t+1$). For the case $t'=t$, we invoke Lemma \ref{lm::probpart} with $l=b/2^{r+2}$, and obtain $\BC_{s/2}(X,Y) \subseteq \BC_{s}(\A)$ with %
	$\tfrac{\eta}{20 \cdot 2^t}$ probability, and since we have $2^t \cdot m$ such clusters, we generate with high probability a pair $(\A,s)$ as above in $\GC_t$.
	We now set $\WC_{t}^\eta = \WC_{t-1}^\eta \cup \WC_\FC^\eta$ and similarly for $\HC_{t}^\eta$.
	We therefore have inductive assumption (1) by counting and (2) by Lemma \ref{lm:reps}. We can therefore conclude by induction that for %
	step $t = \tilde{O}(1)$, we have $\WC^\eta \subseteq \WC$ and $\HC^\eta \subseteq \HC$ as above, and whenever an anchor will be sampled which is in the same ball with both $X$ and $Y$ and close to both of them, $X$ and $Y$ will be clustered together with such anchor, and we can bound $(X,Y) \in [\WC_w \setminus \WC^\eta] \times [\HC_w \setminus \HC^\eta]$ cost as needed.
	\end{proof}


We now present our proof for Lemma \ref{lm::probpart}.

\begin{proof}[Proof of Lemma \ref{lm::probpart}]

Let $\MC_{c}^*$ be a $2c$-matchable set with the properties of Definition \ref{def::dense-in-R}.
Let $t$ be such that $d^{\MC_c^*}_{2c}(\MC_c^*) \in [2^{t-r},2^{t-r+1}]$. Let $A \sim \WC_w$ be a sampled anchor. Let $(\A,s)$ be the output of \textsc{ClusterAnchor} with anchor $A$ at step $t$ as above.

We will argue that with $\tfrac{\eta l}{5 \cdot b \cdot 2^{t-r}}$ probability, $\MC_c^* \cap \A$ contains both $X^* \in \BC_{s/2}(X)$ and $Y^* \in \BC_{s/2}(Y)$. The Lemma immediately follows the claim above, since $\BC_{s/2}(X,Y) \subseteq \BC_{s}(X^*,Y^*) \subseteq \BC_{s}(\A)$ (where the second step follows the triangle inequality).

The more challenging task is proving the claim.

We first define $Z_A$ as the event an anchor $A \in \NC_{2c}(\MC_c^*) \cap \PC_\FC(\MC_c^*)$ will be sampled:

$$Z_A = A \in \NC_{2c}(\MC_c^*) \cap \PC_\FC(\MC_c^*)$$
Next, we define the events $\MC_c^* \cap \A$ containing $X^* \in \BC_{s/2}(X)$ and $Y^* \in \BC_{s}(Y)$. Let $\A_X = P_{2^{r-t}}(\NC_{2c}(A) \cap \WC_w)$,  $\A_Y = P_{2^{r-t}}(\NC_{4c}(A) \cap \HC_w)$,
\begin{align*}
Z_S &= 2^{t-r} \cdot |\A_X \cup \A_Y|\cdot \max\left\{\normint{X^*-X}, \normint{Y^*-Y}\right\} \leq 2l  \\
Z_X &= \A_X \cap \MC_c^* \neq \emptyset \\
Z_Y &= \A_Y \cap \MC_c^* \neq \emptyset 
\end{align*}


Finally, we define the probability of success:
$$\Pr[\text{success}] \geq  \Pr[Z_A] \cdot \Pr[Z_X, Z_Y,Z_S | Z_A] \geq \Pr[Z_A] \cdot (\Pr[Z_X | Z_A] \cdot \Pr[Z_Y | Z_A] - \Pr[\neg Z_S|Z_A])$$

Where the last part is true since $Z_X|Z_A$ and $Z_Y|Z_A$ are either independent or positively correlated and the union bound.

\ns{I guess there is over-notation at this point, and I also think I may have simplification for some of this. will clean up later}

Now, by Fact \ref{fact::setdense} $|\NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)| = \tfrac{|\MC_c^*|\cdot d^{\FC}_{2c}(\MC_c^*)}{d^{\MC_c^*}_{2c}(\MC_c^*)} \geq \tfrac{\eta w l}{2^{t-r+1}}$ %
, we have, 
$$\Pr[Z_A] \geq \tfrac{|\NC_{2c}(\MC_c^*) \cap \FC(\MC_c^*)|}{n} \geq \tfrac{\eta w l}{n \cdot 2^{t-r+1}}$$


Conditioned on finding such anchor, we have:
$$\Pr[Z_X | Z_A] = \Pr[Z_Y | Z_A] = 1- (1-2^{r-t})^{d^{\MC_c^*}_{2c}(\MC_c^*)} \geq 1- \exp(-2^{t-r} \cdot 2^{r-t}) = 1-e^{-1} > 0.63$$
(noting that since $\MC_c^*$ is a ``matchable'' set, then all neighborhoods contains the same amount of $x$-axis and $y$-axis intervals). 

Finally, since for all $(X^*,Y^*)$ matches in $\MC_c^*$, $d_{4c}^{\FC}(Y^*) \cdot \max\{\normint{X^* - X},\normint{Y^* - Y}\} \leq l$, and we sub-sample with prob. $2^{r-t}$, then by the Chernoff bound for $|\FC(A)| = \omega(2^{t-r})$ we have $\Pr[\neg Z_S|Z_A] = o(1)$. We can conclude the probability of success is 
$$\Pr[\text{success}] \geq \tfrac{(0.63^2 - o(1)) \cdot \eta w l }{n \cdot 2^{t-r+1}} > \tfrac{\eta \cdot w \cdot l }{5 \cdot n \cdot 2^{t-r}}$$

as needed.

\ns{IMPORTANT! since we match $y$-axis which can be $4c$-close (rather than $2c$), we actually might end up with larger cluster than the density of $2c$-neighborhood. in other words, the properties of Definition \ref{def::dense-in-R} might be insufficient. When we compound approximations, this becomes even larger problem, but since those are all constants, I believe (hope) this is solvable. For example, one idea would be to use the lowest approximation in which the difference in densities is at most $n^\epsilon$, and just sample more anchors, but this may create exponential dependency in our approximation. }


\end{proof}


==> matching-complexity.tex <==

a_s

\subsection{Complexity}


Now, we claim near-linear complexity. First, we claim that color assignment takes near-linear time. This is essentially true since the sum of $\norm{\psi^l_\kappa(I)}_0$ (over intervals in $\RC^{l}_\kappa$) is at most $\tO(n \cdot \beta)$ at any level $l$.

\begin{lemma}
	Assigning colors in \textsc{ColorIntervals} costs $\tilde{O}(n \cdot \beta)$ time in each level $l$.
\end{lemma}

\begin{proof}
Note that $\sum_{I \in \RC_\kappa^l} \tfrac{ \sum_\chi \phi_\kappa^\chi(\Lambda_\kappa^\zeta(I))}{\beta^l} \leq 2\sum_{I \in \RC_\kappa^l} \sum_\chi \phi_\kappa^\chi(I) \leq 2n$ and hence $\sum_{I \in \RC_\kappa^l} \norm{\psi_\kappa^l(I)}_0 = O(n \cdot \beta \cdot \log^2 n)$ (as we set to 0 any color with weighted potential smaller than $\tfrac{1}{\beta \log^3 n}$). Since WMH costs $\norm{\psi_\kappa^l(I)}_0$ time for each interval, the claim follows.
\end{proof}

Second, we claim that partitions are small.

\begin{lemma}\label{lm::partition_size_new}
	Fix $t \in [\log_\lambda n]$. Each color $\chi \neq -1$ in each coloring
        $\kappa \in \Kappa$ is assigned to at most $ n \cdot \tO_\eps(\beta \cdot \lambda^{-t})$
        intervals (ie, that's the max size of a part in partition).
\end{lemma}
\begin{proof}
	Consider a color $\chi$. Similarly to the above, we have $\sum_{I \in \RC_\kappa^l} \tfrac{ \phi_\kappa^\chi(\Lambda_\kappa^\zeta(I))}{\beta^l} \leq 2\sum_{I \in \RC_\kappa^l} \phi_\kappa^\chi(I) \leq 2n / \lambda^t$, and since we set to 0 any color with weighted potential smaller than $\tfrac{1}{\beta \log^3 n}$, we have that $\chi$ exists on the palette of at most $\tO(n\beta / \lambda^t)$ intervals.
	
	
	
	It remains to show for color $0$, i.e. intervals we did not color. 
	
	
	We now make the following inductive claim.
	
	\begin{claim}
	Fix a level $l$. Consider partitions $\UC^\XC_1,\ldots$ of $\RC_\kappa^l \cap \XC$ and $\UC^\YC_1,\ldots$ of $\RC_\kappa^l \cap \YC$, such that $\UC^\XC_1$ contains the first $\beta^l$ elements of 	$\RC_\kappa^l \cap \XC$, $\UC^\XC_2$ contains the next $\beta^l$ elements and so on. Let $\QC^\XC_1,\ldots,\QC^\YC_1,\ldots$ be the (disjoint) smallest enclosing balls of $\UC^\XC_1,\ldots,\UC^\YC_1,\ldots$.%
	Consider a (corresponding) $\UC, \QC$, which are not at the border. We have one of the following claims whp:
	\begin{enumerate}
		\item For all $I \in \UC$, $I$ will be colored and hence, $\QC \cap \RC_\kappa^{l+1} = \emptyset$; or
		\item the number of intervals $I \in \QC$ with relative density $d_{c, Q, \kappa}(I) = O(\tfrac{N \cdot \log n}{\epsilon \beta^l \cdot \lambda^t})$ is at least $(1-\tfrac{(l+1) \cdot \epsilon}{2}) \cdot \beta^l$.
	\end{enumerate}

	\end{claim}	
	\begin{proof}
	We prove by induction $l$. When $l=0$ ($\beta^l=1$), if density of an interval $I$, $d_{c,\{I\},\kappa}(I) \geq O(\tfrac{N \log n}{\lambda^t})$, then for each color $\chi$, $\phi_\kappa^\chi(I)$ is a r.v. bounded by $1/\log n$ and expectation $\lambda^{-t}$, and since we sample $\lambda^t$ i.i.d anchors, $\sum_\chi \phi_\kappa^\chi(I)$ will concentrate around its expectation $\approx 1$ and hence we will mark such interval with $-1$ whp. %
	Consider a non-border set $\QC$ at level $l$ with apriori $\beta^l$ uncolored intervals. %
	We observe that $\QC$ must contain at least $\beta-3$ complete sets $\QC'$ from level $l-1$ where the corresponding $\UC'$ was not fully colored, and hence by inductive hypothesis, $\QC$ contains $(1-\tfrac{l \cdot \epsilon}{2}) \cdot (\beta-3)\beta^{l-1} \geq (1-\tfrac{l \cdot \epsilon}{2} - \tfrac{\epsilon}{50})\cdot \beta^{l}$
	intervals with relative density $d_{c, \QC, \kappa}(I) = O(\tfrac{N \cdot \beta \cdot \log n}{\epsilon \beta^l \cdot \lambda^t})$.
	  %
	Now, consider 2 cases when coloring level $l$. In the below, note relative density of interval is monotonically decreasing as we go up the tree.%
	
	\begin{enumerate}
		
		\item If there exists a set of intervals $\CD \subseteq \QC$ of size $|\CD|=\tfrac{\epsilon}{3} \cdot \beta^l$, such that for each $I \in \CD$ we have $d_{c, \QC, \kappa}(I) \in \tfrac{N}{\beta^l \cdot \lambda^t} \cdot [O(\tfrac{\log n}{\epsilon}),\beta \log^2 n]$, we invoke Lemma \ref{lm::dense_set} and obtain that whp, $\normo{\varphi_\kappa^l(\QC)} \geq \tfrac{\epsilon}{4} > T$. 
	
				Now, consider an interval $I \in \UC$.
 Since $\QC \subseteq \Lambda_\kappa^\zeta(I)$ (for any $I \in \UC$ and any $\zeta \geq \beta^l$), then we have $\normo{\psi_\kappa^l(I)} > T$ and hence the color $0$ will not appear on the {\em palette} of $I$, and $I$ must therefore be colored (with high probability). %
				
		
		\item Otherwise, we have $(1-\tfrac{l \cdot \epsilon}{2} - \tfrac{\epsilon}{50} - \tfrac{\epsilon}{3}) \cdot \beta^l > (1-\tfrac{(l+1) \cdot \epsilon}{2}) \cdot \beta^l$ intervals with relative density $d_{c, \QC, \kappa}(I) = O(\tfrac{N \log n}{\epsilon \beta^l \cdot \lambda^t})$ %
		, and the claim follows.
	\end{enumerate}
	We have therefore proved the inductive assumption continues to hold at the end of level $l$ as well. This concludes the proof of the claim.
	\end{proof}
	
	Note that since each interval has density at least $1$, this proves that where we are done at level $\bar{l} \leq 1/\epsilon$, $|\RC_\kappa^{\bar{l}}| \leq \beta^{\bar{l}} \leq \tO(\tfrac{\beta N \log n}{\lambda^t})$ as needed.
\end{proof}



==> matching-correctness.tex <==
\subsection{Correctness}

Fix an alignment $\pi: \XC \rightarrow \YC \cup \{ \bot \}$. We define the {\em extension of $\pi$}, $\widehat{\pi}: \IC \rightarrow \IC \cup \{ \bot \}$, such that,

$$\widehat{\pi}[I] = \begin{cases}
\pi[I] & I \in \XC \\
\pi^{-1}[I] & I \in \YC
\end{cases}$$

For the rest of this section, when we mention an alignment $\pi$, we loosely refer to its extension.
We also define,

\begin{definition}[Corrupted interval - new]
	Fix $w \in \N$, alignment $\pi \in \Pi$, and coloring $\kappa$. Then an interval $I \in \IC_w$ is
        a {\em $(\kappa,\pi,c)$-corrupted interval} if either
        \begin{enumerate}
       \item $\pi(I)=\bot$;
       \item $\cad(I,\pi[I]) > c$; or
        \item $I \not\equiv_\kappa \pi[I]$.
      \end{enumerate}
\end{definition}





We define the set $\EC_\kappa \subseteq \IC$ as the subset of {\em $(\kappa,\pi,c)$-corrupted intervals}.

Finally, we define a measurement $\rho_\kappa^l(I)$ to capture the ``corruptness'' of an interval ball with respect to the number of uncolored intervals as follows, $\rho_\kappa^l(I) = \tfrac{|\Lambda_\kappa^{\bar{\zeta}}(I) \cap \EC_\kappa|}{\beta^l}$, where $\bar{\zeta} = \max(\zeta) < 2\beta^l$.



Our main correctness claims follow.

First, we derive the total ``corruptness'' of uncolored intervals is proportional to the number of corrupted intervals.
\begin{lemma}\label{lm::rho_bound_new}
	Fix $\kappa, l, n, \RC^{l}_\kappa$. We have that $\sum_{I \in \RC^{l}_\kappa} \rho_\kappa^l(I) = O(|\EC_\kappa|)$.
\end{lemma}

\begin{proof}
	$$\sum_{I \in \RC_\kappa^l} \frac{|\Lambda_\kappa^{\bar\zeta}(I) \cap \EC_\kappa|}{\beta^l} \leq \sum_{I' \in \EC_\kappa} \frac{|\Lambda_\kappa^{\bar\zeta}(I') \cap \RC_\kappa^l|}{\beta^l} \leq \sum_{I' \in \EC_\kappa} \frac{4\beta^l}{\beta^l} = O(|\EC_\kappa|)$$.
\end{proof}

Next, we show that the expected $\ell1$ distance the palettes of intervals and their corresponding intervals in $\pi$ is bounded by their ``corruptness'' parameter.


First we show the following combinatorial lemma.



\begin{lemma}\label{lm::bound_delta_psi}
	Fix $T,\rho > 0$ and $k,n \in \N$ with $k < n$. Fix $v_1,\ldots,v_n$ and $u_1,\ldots,u_n$, each a non-negative, monotonically increasing, bounded series of vectors sampled from some (common) probability space, such that $\normo{v_i},\normo{u_i} \leq T$. In addition, we have that for any $i$, there exists a r.v. $\widehat{u_i}$, such that,
	\begin{itemize}
		\item $u_{i-k} \leq \widehat{u_i} \leq u_{i+k}$; and
		\item $\E[\normo{v_i - \widehat{u_i} }] \leq \rho$.
	\end{itemize}
	Then,	
	$$
	\E_{i \in [n]} \left[\E\left[\normo{v_i - u_i}\right]\right] = O(\rho + \tfrac{k \cdot T}{n}).
	$$
\end{lemma}
\begin{proof}
By triangle inequality we get
$$\sum_{i \in [n]} \E\left[\normo{v_i - u_i}\right] \leq \sum_{i \in [n-2k] + k} \E\left[\normo{v_i - \widehat{u_i}}\right] + \sum_{i \in [n-2k] + k} \E\left[\normo{\widehat{u_i} - u_i}\right] + 2kT$$

From the second promise we can bound the first term: $\sum_{i \in [n-2k] + k} \E\left[\normo{v_i - \widehat{u_i}}\right] \leq \rho n$.



It remains to bound the second term: $\sum_{i \in [n-2k] + k} \E\left[\normo{\widehat{u_i} - u_i}\right]$.

\begin{align*}
	\sum_{i \in [n-2k] + k} \E\left[\normo{\widehat{u_i} - u_i}\right] &\leq \sum_{i \in [n-2k] + k} \max_{j \in \{-k,k\}}\E\left[\normo{u_{i+j} - u_i}\right] \\
		&\leq 2\sum_{i \in [n-k]} \E\left[\normo{u_{i+k} - u_i}\right] \\
		&\leq 2\sum_{i \in [n-k]} \E\left[ \sum_{j \in [k]} \normo{u_{i+j} - u_{i+j-1}}\right] \\
		&\leq 2k\sum_{i \in [n-1]}\E\left[\normo{u_{i+1} - u_i}\right]\\
		&\leq 2k T
	\end{align*}
	Where the first and last inequalities are by monotonicity of $b$ and the 3rd is by applying triangle inequality. since $\E_{i \in [n]} \left[\E\left[\normo{v_i - u_i}\right]\right] = \tfrac{1}{n}\sum_{i \in [n]} \E\left[\normo{v_i - u_i}\right]$, we obtain the statement.
\end{proof}



\begin{lemma}\label{lm::ham_dist_new}
	Fix $t,c,w,l \in \N$, %
	alignment
        function $\pi \in \Pi$. Fix input coloring $\kappa'$ and remaining set $\RC^{l}_{\kappa}$ for some output coloring $\kappa$ at step $t$. Consider $I \in \RC^{l}_{\kappa}$, and fix $\rho= \rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])$.

	Consider same-diameter balls $\BC_I \subseteq \Lambda_\kappa^{\bar\zeta}(I), \BC_{\pi[I]} \subseteq \Lambda_\kappa^{\bar\zeta}(\pi[I])$, where $I$, $\pi[I]$ are in the same exact respective position w.r.t $\BC_I,\BC_{\pi[I]}$.
	
     Then we have by expectation (over the random choice of anchors), that, 
     $$\E\left[\normo{\varphi_\kappa^l(\BC_I) - \varphi_\kappa^l(\BC_{\pi[I]})}\right] = O(\rho)$$.

\end{lemma}

\begin{proof}
Let $\gamma = \tfrac{1}{\beta \log^2 n}$,
 $p_\chi=\sum_{I' \in \BC_I}\phi_\kappa^\chi(I')$ and
$q_\chi=\sum_{I' \in \BC_{\pi[I]}}\phi_\kappa^\chi(I')$.
Then, we can rewrite the $\ell_1$ norm as:

$$                \sum_\chi \left| \max
                \left\{\tfrac{p_\chi}{\beta^l},\gamma\right\} - \max
                \left\{\tfrac{q_\chi}{\beta^l},\gamma\right\} \right| 
\le                 \beta^{-l} \cdot \sum_\chi \left| p_\chi-q_\chi\right|.
$$

It remains to compute (the expected value of) $\sum_\chi \left|
p_\chi-q_\chi\right|$, i.e., expected difference in potential. 
Let us count the expected potential distance for any fixed color. We note that if an interval
 $I' \in \BC_I \cup \BC_{\pi[I]}$ 
 is matched to some anchor $A$, and $I'$ is not {\em $(\kappa',\pi,c)$-corrupted interval}, then the same potential will be added to $\pi[I']$ (assuming perfect neighborhoods). Hence the potential distance can be generated from either corrupted intervals, or intervals  $I' \in \BC_I \cup \BC_{\pi[I]}$  where $\pi[I']$ is not in the corresponding ball.
    
    Since $\rho \geq \rho_\kappa^l(I') + \rho_\kappa^l(\pi[I'])$, then there exists at most $O(\rho \beta^l)$ corrupted intervals in the balls. Furthermore, the number of ball ``mismatches'' (i.e. where $I'$ in ball, but $\pi[I']$ not in corresponding ball) is bounded by $O(\rho \beta^l)$ as well (for each interval mismatch there is a unique corrupted interval $I''$ where $\pi[I'']=\bot$).%
    
    We therefore conclude that the potential distance is bounded by potential generated from a subset of $O(\rho \beta^l)$ intervals. %
    
    Since the expected potential of each interval is precisely 1, we get:
    $$
    \E\left[ \sum_\chi \left| \max
                \left\{\tfrac{p_\chi}{\beta^l},\gamma\right\} - \max
                \left\{\tfrac{q_\chi}{\beta^l},\gamma\right\} \right|\right]
    \leq \beta^{-l} \cdot \E\left[\sum_\chi \left| p_\chi-q_\chi\right|\right] \\
    = \beta^{-l} \cdot O(\rho \beta^l) = O(\rho).
    $$.
    completing the proof.

\end{proof}

As a result, we can bound the corruption growth each level.

\begin{lemma}\label{lm::corruption_growth}
	Fix $t,c,w \in \N$, $\eps \in [0,1]$, alignment
        function $\pi \in \Pi$. Fix level $l$ with input coloring $\kappa'$ and output coloring $\kappa$.%
        Let $k=|\EC_{\kappa'} \cup \EC_{\kappa}|$ be the number of expensive interval at level $l$.
          Then, \textsc{ColorIntervals} at level $l$ colors $\kappa$ such that at the next level we have that $|\EC_{\kappa'} \cup \EC_{\kappa}| = O(\tfrac{k}{\epsilon \cdot \eta})$ %
         with probability $1-\eta$.
\end{lemma}

The proof is provided in the next section.

Finally, we derive,

\begin{lemma}\label{lm::existence_good_color}
	Fix $t,c,w \in \N$, $\eps$, alignment
        function $\pi \in \Pi$. Suppose we call to \textsc{MatchIntervals} at step $t$ with coloring $\kappa$. %
          Then with high probability, we generate  a coloring $\kappa' \in \Kappa$ where $|\EC_{\kappa'}| = O(\epsilon)^{-2/\epsilon} \cdot |\EC_{\kappa}|$.        %
\end{lemma}
\begin{proof}
	Fix a coloring $\kappa_j$. From Lemma \ref{lm::corruption_growth}, at each level $l \in [\log_\beta n]$ we have $O(\epsilon^{-2})$ factor growth in corruption with probability $1-\epsilon/2$, and by the union bound we get overall blow-up $O(\epsilon)^{-2/\epsilon}$ with probability $1/2$ (as we have $1/\epsilon$ levels). Since generate $O(\log n)$ i.i.d colorings, the claim follows.
\end{proof}

\ns{Actually, I think we don't need union bound / markov as the corruption growth r.v. are independent, hence we can show the expectation of product is product of expectations, and we save some factor in exponent.}


\subsection{Proof of Lemma \ref{lm::corruption_growth}}
\begin{proof}[Proof of Lemma \ref{lm::corruption_growth}]



Fix level $l$, and consider an {\em uncorrupted interval} $I \in \RC^{l}_\kappa \setminus \EC_\kappa \setminus \EC_{\kappa'}$. We show that the probability to {\em corrupt} $I$ is bounded by $O(\rho/\epsilon)$, where $\rho = \rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])$. Note that if $\rho \geq \tfrac{\epsilon}{100}$ the statement is trivial, so we assume $\rho < \tfrac{\epsilon}{100}$. %

	Note that the only way to corrupt $I$ at level $l$ is by having $I$ and $\pi[I]$ contain different colors at the end of level $l$.
	
	Since we assign $\kappa(I) = h(\psi_\kappa^l(I)), \kappa(\pi[I]) = h(\psi_\kappa^l(\pi[I]))$ using WMH function, then by Theorem \ref{?}, the probability of collision is $1-\tfrac{\normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}}{\normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])}} \geq 1-\tfrac{\normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}}{T} = 1 - O(\tfrac{1}{\epsilon}) \cdot \normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}$.
	
	It remain to bound the quantity $\normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}$.
	
	Now consider a ball $\LC_I^\zeta$ on the left $I$ defined by parameter $\zeta \in [1,1+\tfrac{\epsilon}{100}] \cdot \beta^l \cap \N$ of uncolored intervals on the left, which is sampled randomly from the range, and let $L_i(I)$ and $L_i(\pi[I])$, respectively, be the potential vectors $\varphi^l_\kappa(\LC_I^\zeta)$ and $\varphi^l_\kappa(\LC_{\pi[I]}^\zeta)$, capped at total potential $T$ as described earlier. Similarly, let $R_i(I)$ and $R_i(\pi[I])$ be the potential vectors on the right.
	
	We note that since there are at most $\rho \cdot \beta^l$ corrupted intervals within $\Lambda_\kappa^{\beta^l}(I) \cup \Lambda_\kappa^{\beta^l}(\pi[I])$, then $|\LC_{\pi[I]}^{\zeta - \rho \beta^l}| \leq |\LC_I^\zeta| \leq |\LC_{\pi[I]}^{\zeta + \rho \beta^l}|$, and hence there exists a set $\widehat{\LC_{\pi[I]}^{\zeta}}$  such that $\LC_{\pi[I]}^{\zeta - \rho \beta^l} \subseteq \widehat{\LC_{\pi[I]}^{\zeta}} \subseteq \LC_{\pi[I]}^{\zeta + \rho \beta^l}$, with $|\widehat{\LC_{\pi[I]}^{\zeta}}| = |\LC_I^\zeta|$. Let $\widehat{L_i} = \varphi^l_\kappa(\widehat{\LC_{\pi[I]}^{\zeta}})$, capped at $T$. We invoke Lemma \ref{lm::ham_dist_new} and obtain that $\E\left[\normo{L_i(I) - \widehat{L_i}}\right] = O(\rho)$ (nothing that capping both potentials at any threshold $T$ can increase the distance by factor 2 at most). \ns{need to formally argue this in previous lemma.} 
	
	We now use Lemma \ref{lm::bound_delta_psi}, setting $v_i = L_i(I), u_i = L_i(\pi[I]), \widehat{u_i}=\widehat{L_i}$
	, $n=\tfrac{\epsilon}{100} \cdot \beta^l, k= \rho \cdot \beta^l$, and $T=\tfrac{\epsilon}{100}$, 
	to obtain $\E\left[\normo{L_i(I) - L_i(\pi[I])}\right] = O(\rho)$ as well. We derive by similar analysis on the right that $\E\left[\normo{R_i(I) - R_i(\pi[I])}\right] = O(\rho)$, and hence by Fact \ref{ft::psi_distance_lr} we obtain
	
	$$\E\left[\normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}\right] \leq \E\left[2 \left(\normo{L_i(I) - L_i(\pi[I])} + \normo{R_i(I) - R_i(\pi[I])}\right)\right] = O(\rho)$$
	
	 as well. We therefore conclude the probability $I$ and $\pi[I]$ will not collide is bounded by $O(\tfrac{\rho}{\epsilon})$.


	
	
	Second, summing over all $I \in \RC_\kappa^l$, we use Lemma \ref{lm::rho_bound} to bound the expected number of newly corrupted intervals.
	$$\E [\text{newly corrupted intervals}] = \sum_{I \in \RC^{l}_\kappa} \Pr[\text{corrupt } I] = \sum_{I \in \RC^{l}_\kappa} O(\tfrac{\rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])}{\epsilon}) = O(\tfrac{|\EC_\kappa \cup \EC_{\kappa'}|}{\epsilon}).$$
	
	
	The soundness of the Lemma follows the Markov inequality.
\end{proof}


==> matching.tex <==
\section{New Analysis}

We adjust slightly the algorithm by redefining balls for coloring. Instead of using fixed radius balls $\BC_{s}(I)$ around $I$, %
we look at the smallest enclosing ball containing $s$ intervals in $\RC_\kappa^l$ closest to $I$ on the left, and similarly on the right. We define $\Lambda_\kappa^\zeta(I)$ as the smallest interval ball containing $\zeta$ intervals on each side in $\RC_\kappa^l$ as above. \ns{formalize better.}


Next, we define $\varphi$ scores for set $\SC$ as,
$$(\varphi^l_\kappa(\SC))_\chi = \max \left(\frac{\phi_{\kappa}^\chi(\SC)}{\beta^l} - \tfrac{1}{\beta \log^3 n},0\right)$$

Fix a threshold $T = \tfrac{\epsilon}{100}$ and integer $\zeta \in [1,1+\tfrac{\epsilon}{100}] \cdot \beta^l \cap \N$ (which would be sampled uniformly within the range), we build the $\psi^l_\kappa(I)$ vector as follows. We count the potential $\varphi^l_\kappa(\LC)$, for the largest subset $\LC \subseteq \Lambda_\kappa^\zeta(I)$ on the left of $I$ with $\normo{\varphi^l_\kappa(\LC)} < T$. Then, we add part of the potential of the next interval on the left of $\LC$ (if such exists within $\Lambda_\kappa^\zeta(I)$) so we reach precisely $T$ potential score (pro-rated if there is more than 1 color). We perform the same calculation on the right of $I$, and define $\psi_\kappa^l(I)$ to be the sum of potentials on the left and on the right using the process above. If the total potential is less than $T$ then we add color $0$ to $\psi_\kappa^l(I)$ so that $\normo{\psi_\kappa^l(I)} = T$ precisely. Note that $\normo{\psi_\kappa^l(I)} \in [T,2T]$.

\ns{show we can perform such process efficiently.}

In addition, we do not use a threshold test now, but apply WMH on all intervals. Note, however, that since we add the color $0$ to the $\psi$, we still have some intervals remaining uncolored in each level as before.

\begin{fact}\label{ft::psi_distance_lr}
	Fix, $I, I', l, \kappa$. Let $L(I), R(I)$ represent the potential vectors on the left and on the right as defined above, and similarly for $L(I'), R(I')$. We have that,
$$\normo{\psi_\kappa^l(I) - \psi_\kappa^l(I')} \leq 2 \left(\normo{L(I) - L(I')} + \normo{R(I) - R(I')}\right)$$
\end{fact}
\begin{proof}
	By triangle inequality, we get
\begin{align*}
	\normo{\psi_\kappa^l(I) - \psi_\kappa^l(I')} &= \normo{L(I) + R(I) - (L(I') + R(I'))} + | \normo{L(I) + R(I)} - \normo{L(I') + R(I')} | \\
	&\leq 2\normo{L(I) + R(I) - (L(I') + R(I'))} \\
	&\leq 2 \left(\normo{L(I) - L(I')} + \normo{R(I) - R(I')}\right)
\end{align*}


\end{proof}
Also, we let $N = |S| \leq n$, i.e. the number of not {\em already matched} intervals, and assume we assign score $\tfrac{N}{|\A| \cdot \lambda^t}$ for matched intervals (instead of $\tfrac{n}{|\A| \cdot \lambda^t}$).

Finally, we stop coloring at level $\bar{l} \leq 1/\epsilon$ when $|\RC_\kappa^{\bar{l}}| \leq \beta^{\bar{l}}$.

\subsection{Relative Density}
We use the following definition.
	\begin{definition}[Relative Density]
		Fix $I \in \IC$, $\kappa$, cost $c$ and an interval set $\SC$. The relative density $d_{c, \SC, \kappa}(I)$ is the relative size of neighborhood of $I$ in partition $\PC_\kappa$ divided by such neighborhood when restricted to the set $\SC$, ie
		$$d_{c, \SC, \kappa}(I) = \tfrac{|\NC_c(I) \cap \PC_\kappa(I)|}{|\NC_c(I) \cap \PC_\kappa(I) \cap \SC|}$$.
	\end{definition}
	
	Note that $d_{c, \SC, \kappa}(I) \geq 1$ and is monotonically decreasing in $\SC$. We also note the following fact about dense sets.
	\begin{fact}\label{ft::rel_dense_bound}
		Fix interval $I$, interval set $\SC$, color $\chi$, and step $t$. Let $d=d_{c,\SC,\kappa}(I)$. Then $\phi^\chi_\kappa(I) > 0 \Rightarrow \phi^\chi_\kappa(\SC) = \tfrac{N}{d \cdot \lambda^t}$.	\end{fact}

\begin{proof}
	Since we assume perfect neighborhood and $I$ is a match, then
	$$\phi^\chi_\kappa(\SC) = \sum_{I' \in \NC_c(I) \cap \PC_\kappa(I) \cap \SC} \phi^\chi_\kappa(I') = \sum_{I' \in \NC_c(I) \cap \PC_\kappa(I) \cap \SC}\tfrac{N}{|\NC_c(I) \cap \PC_\kappa(I)| \cdot \lambda^t} = \tfrac{N \cdot |\NC_c(I) \cap \PC_\kappa(I) \cap \SC|}{|\NC_c(I) \cap \PC_\kappa(I)| \cdot \lambda^t} = \tfrac{N}{d \cdot \lambda^t}.$$
\end{proof}
	
	
We now claim the following Lemma which will later help us show if we have a set with the ``right'' density within some ball $\QC$, then we color all uncolored intervals in $\QC$ whp. 

\begin{lemma}\label{lm::dense_set}
	Fix a constant $\delta > 0$. Fix sets $\CD, \QC$ with $\CD \subseteq \QC \subseteq \IC$ and $|\CD| = \delta \cdot \beta^l$. Assume further than for all $I \in \CD$, we have $d_{c,\QC,\kappa}(I) \in \tfrac{N}{\beta^l \lambda^t} \cdot [O(\tfrac{\log n}{\delta}),\beta \cdot \log^2 n]$. Then, with high probability, we have at step $l$,
	$$\normo{\varphi^l_\kappa(\QC)} \geq 0.9 \delta$$
\end{lemma}
\begin{proof}
	For any interval $I \in \CD$, and any color $\chi$, we have $\E[\phi^\chi_\kappa(I)] = \lambda^{-t}$, and hence we have $\E[\phi^\chi_\kappa(\CD)] = \delta \cdot \beta^l \cdot \lambda^{-t}$.
	Now, on one hand, since $d_{c,\CD,\kappa}(I) \geq d_{c,\QC,\kappa}(I) \geq \tfrac{N}{\beta^l \lambda^t} \cdot O(\tfrac{\log n}{\delta})$, then by Fact \ref{ft::rel_dense_bound} we have $\phi^\chi_\kappa(\CD) \leq \tfrac{\delta}{O(\log n)} \cdot \beta^l$. Therefore, the quantity $\sum_\chi \phi^\chi_\kappa(\CD)$ can be seen as a sum of $\lambda^t$ iid r.v. with expectation $\delta \cdot \beta^l \cdot \lambda^{-t}$ and bounded by $\tfrac{\delta \beta^l}{O(\log n)}$. Therefore, by Bernstein concentration inequality, we obtain whp $\sum_\chi \phi^\chi_\kappa(\CD) \in [0.95,1.05]\E[\sum_\chi \phi^\chi_\kappa(\CD)] = [0.95,1.05]\delta \beta^l$. On the other hand, since $d_{c,\QC,\kappa}(I) \leq \tfrac{N}{\beta^l \lambda^t} \cdot \beta \log^2 n$, then assuming $\phi^\chi_\kappa(\CD) > 0$, we have $\phi^\chi_\kappa(\QC) > \tfrac{\beta^l}{\beta \log^2 n}$, and hence $(\varphi^l_\kappa(\QC))_\chi \geq \phi^\chi_\kappa(\QC) \cdot \beta^{-l} - \tfrac{1}{\beta \log^3 n} \geq (1-\tfrac{1}{\log n}) \cdot \phi^\chi_\kappa(\QC) \cdot \beta^{-l}$.  Summing over all such coordinates, we obtain the following bound with high probability,
	$$\sum_{\chi:\phi^\chi_\kappa(\CD) > 0} (\varphi^l_\kappa(\QC))_\chi \geq (1-o(1))\sum_{\chi:\phi^\chi_\kappa(\CD) > 0} \phi^\chi_\kappa(\QC) \cdot \beta^{-l} \geq (1-o(1))\sum_{\chi} \phi^\chi_\kappa(\CD) \cdot \beta^{-l}> 0.9\E[\sum_\chi \phi^\chi_\kappa(\CD)] \cdot \beta^{-l} = 0.9 \delta$$
	which implies,
	$$\normo{\varphi^l_\kappa(\QC)} =  \sum_{\chi} (\varphi^l_\kappa(\QC))_\chi \geq \sum_{\chi:\phi^\chi_\kappa(\CD) > 0} (\varphi^l_\kappa(\QC))_\chi \geq 0.9 \delta$$
	with high probability as well, as needed.
\end{proof}

\subsection{Algorithm}
In the below, $T \gets \tfrac{\epsilon}{100}$, $\psi$ is also a function of $T,\zeta$.

\begin{algorithm}[H]
\caption{Matching Phase - Color Intervals}
\begin{algorithmic}[1]
\label{alg::matching.color_new}
\Function{ColorIntervals}{$\RC^l_\kappa,\kappa,l$}
\State Sample $\zeta%
\sim [1,1+\tfrac{\epsilon}{100}]\beta^l \cap \N$ uniformly.

\State Sample  %
 WMH function $h$.
\State Compute all
$\psi^l_\kappa(I)$ for 
$I \in \RC^{l}_\kappa$ as above.

      	\For {$I \in \RC^{l}_\kappa$}
    		\State  $\kappa(I) \gets \begin{cases} 
      -1 & l=0 \\
      h(\psi^l_\kappa(I)) & l>0
   \end{cases}$
      		 %
        \EndFor
        \State \Return $\kappa$.
\EndFunction	
\end{algorithmic}
\end{algorithm}


In the below, we make an initial call with:
\begin{enumerate}
	\item $t \gets 1 .\SC \gets \IC$.
	\item $\forall I\in \IC, \kappa(I) \gets 0$.
\end{enumerate}

\begin{algorithm}[H]
\caption{Matching Phase}
\begin{algorithmic}[1]
\label{alg::matching.new2}	

\Function{MatchIntervals}{$\SC, \GC_w, c, \kappa,t$}
				\State Initialize $\Kappa = \{\kappa_1,\ldots,\kappa_m\}$.
				
				\State $G \gets$ unweighted and undirected graph with nodes $I \in \IC$ and no edges. 

				 
				\For {$j \in [m]$}  
				\For {$l \in 0\ldots \log_\beta n$}
					\State $\phi_{\kappa_j} \gets \vec{0}$.%

					\For {$\chi \in [\lambda^t]
                                  $}
				\State Sample $A%
				\sim \SC$ uniformly at random.%
				\State $\A%
				\gets $ \textsc{ClusterAnchor}($A,\PC_{\kappa}(A), \GC_w, c$).
				\State Add edges $(A,I)$ for $I \in \A$ to $G$.
				\State $\textsc{AssignPotential}(\A,A,\chi,\GC_w, c)$.
				\EndFor
						\State $\RC^{l}_{\kappa_j} \gets \{I \in \SC \mid \kappa_j(I) = 0\}$.
						\State $\kappa_j \gets \textsc{ColorIntervals}(\RC^{l}_{\kappa_j},\kappa_j,l)$.
				\EndFor
				\State $\SC_j \gets \{I \in \SC \mid \kappa_j(I) \neq -1\}$.
			\EndFor
		\State $G \gets \cup_{j 
		\in [m], \SC_j \neq \emptyset} \textsc{MatchIntervals}(\SC_j, \GC_w, c, \kappa_j,t+1)$.
		
	\State \Return $G$.
\EndFunction

\end{algorithmic}
\end{algorithm}


==> newalgo-complexity.tex <==

\subsection{Complexity}

For both Complexity and Correctness, we use the following auxiliary lemma, showing we can allocate ``cost'' of intervals to some other intervals in  an important subset within a certain radius, such that the sum of weighted cost using the same radius preserves the total cost. \ns{phrase better}

\begin{lemma}\label{lm::cost_fg}
	Fix $\SC \subseteq \IC$, cost function $f: \IC \rightarrow \R$ and radius $s$. Let $g: \SC \rightarrow \R$ be a function such that $g(I') = \tfrac{\sum_{I \in \BC_s(I')} f(I)}{|S \cap \BC_s(I')|}$. Then, 
$\sum_{I \in \SC} g(I) = O\left(\sum_{I \in \IC} f(I)\right)$
\end{lemma}

\begin{proof}
	Fix an interval $I \in \IC$. Let $L_I$ be the set of intervals $\BC_{s}(I) \cap \SC$ left of $I$ and $R_I$ be the set of intervals on the right, i.e.
	\begin{align*}
		L_I &= \{I - i\}_{i \in [s]} \cap \SC\\
		R_I &= \{I + i\}_{i \in [s]} \cap \SC
	\end{align*}
	
	 For each interval $I' \in L_I$, we add $\tfrac{f(I)}{|L_I|}$ to $\widehat{g(I')}$. Similarly, for each interval $I' \in R_I$. we add $\tfrac{f(I)}{|R_I|}$ to  $\widehat{g(I')}$. 
	  %
	 Note that on one hand, the total amount added to $\sum_{I' \in \SC} \widehat{g(I')}$ is bounded by $2\sum_{I \in \IC} f(I)$. 
	 On the other hand, $L_I \subseteq \BC_{s}(I') \cap \SC$ for each $I' \in L_I$, and hence $\tfrac{f(I)}{|L_I|} \geq \tfrac{f(I)}{|\BC_{s}(I') \cap \SC|}$ and similarly for intervals in $R_I$. 
	 We can therefore conclude that $\widehat{g(I')} \geq g(I')$ for any $I' \in S$ and hence $\sum_{I \in \SC} g(I) = O\left(\sum_{I \in \IC} f(I)\right)$.
\end{proof}


Now, we claim near-linear complexity. First, we claim that color assignment takes near-linear time. This is essentially true since the sum of $\norm{\psi^l_\kappa(I)}_0$ (over intervals in $\RC^{l}_\kappa$) is at most $\tO(n \cdot \beta)$ at any level $l$.

\begin{lemma}
	Assigning colors in \textsc{ColorIntervals} costs $\tilde{O}(n \cdot \beta)$ time in each level $l$.
\end{lemma}

\begin{proof}
Fix $f(I) = \sum_\chi \phi_\kappa^\chi(I)$, $\SC=\RC_\kappa^l$ and $s = \beta^l$. We invoke Lemma \ref{lm::cost_fg} and obtain $\sum_{I \in \RC_\kappa^l} \tfrac{ \sum_\chi \phi_\kappa^\chi(\BC_\beta^l(I))}{|\BC_\beta^l(I) \cap \RC_\kappa^l|} \leq n$ and hence $\sum_{I \in \RC_\kappa^l} \norm{\psi_\kappa^l(I)}_0 = O(n \cdot \beta \cdot \log^2 n)$ (as we set to 0 any color with weighted potential smaller than $\tfrac{1}{\beta \log^2 n}$). Since WMH costs $\norm{\psi_\kappa^l(I)}_0$ time for each interval, the claim follows.
\end{proof}

Second, we claim that partitions are small.

\begin{lemma}\label{lm::partition_size_new}
	Fix $t \in [\log_\lambda n]$. Each color $\chi \neq -1$ in each coloring
        $\kappa \in \Kappa$ is assigned to at most $ n \cdot \tO_\eps(\beta \cdot \lambda^{-t})$
        intervals (ie, that's the max size of a part in partition).
\end{lemma}
\begin{proof}
	Consider a color $\chi$. Similarly to the above, we set $f(I) = \phi_\kappa^\chi(I)$, $\SC=\RC_\kappa^l$ and $s = \beta^l$. We invoke Lemma \ref{lm::cost_fg} and obtain $\sum_{I \in \RC_\kappa^l} \tfrac{ \phi_\kappa^\chi(\BC_\beta^l(I))}{|\BC_\beta^l(I) \cap \RC_\kappa^l|} \leq n$, and since we set to 0 any color with weighted potential smaller than $\tfrac{1}{\beta \log^2 n}$, we have that $\chi$ exists on the palette of at most $\tO(n\beta / \lambda^t)$ intervals.
	
	
	
	It remains to show for color $0$, i.e. intervals we did not color. For this we make the following definition.
	
	\begin{definition}[Relative Density]
		Fix $I \in \IC$, $\kappa$, cost $c$ and an interval set $\SC$. The relative density $d_{c, \SC, \kappa}(I)$ is the relative size of neighborhood of $I$ in partition $\PC_\kappa$ divided by such neighborhood when restricted to the set $\SC$, ie
		$$d_{c, \SC, \kappa}(I) = \tfrac{|\NC_c(I) \cap \PC_\kappa(I)|}{|\NC_c(I) \cap \PC_\kappa(I) \cap \SC|}$$.
	\end{definition}
	
	Note that $d_{c, \SC, \kappa}(I) \geq 1$ and is monotonically decreasing in $\SC$. 
	
	We also state the following numerical fact.
	
		\begin{fact}\label{ft::sum_adjacent}
		Fix $\alpha,\eta > 0$. Let $e_1,\ldots,e_n$ and $s_1,\ldots,s_n$ be $2n$ non-negative numbers, with the promise that for each $i \in \{2,3,\ldots,n-1\}$, $s_i + \alpha (s_{i-1} + s_{i+1}) \geq (1-\eta)e_i$. Then, we have that $\sum_{i \in [n]} s_i \geq \sum_{i \in \{2,\ldots,n-1\}}(1-\eta - 2\alpha)e_i$
	\end{fact}
	\begin{proof}
	If we sum the above over $i \in \{2,3,\ldots,n-1\}$, we obtain that,
	
	$$ 
	\sum_{i \in \{2,\ldots,n-1\}}(1-\eta)e_i 
	\leq \sum_{i \in \{2,3,\ldots,n-1\}} s_i + \alpha (s_{i-1} + s_{i+1})
	\leq \sum_{i \in [n]} (1+2\alpha)s_i 
	$$
	and since $\alpha,\eta>0$, the claim follows.
	\end{proof}
	
	
	We now make the following inductive claim.
	
	\begin{claim}
	Consider a $\beta$-ary trees $T_\XC$ and $T_\YC$, respectively, over $\XC$ and $\YC$.
		Consider any sub-tree $q \in T_\XC \cup T_\YC$ at level $l$ that has $r=|\RC_\kappa^{l+1} \cap q|$ remaining non-colored intervals at the end of level $l$. Let $s_q$ be the number of intervals $I \in q$ with relative density $d_{c, \BC_{\beta^l}(q), \kappa}(I) = O_\epsilon(\tfrac{n \cdot \log n}{r \cdot \lambda^t})$, and $s_q'$ the number of such intervals in adjacent sub-trees at the same level as $q$. 
		Then $s_q + \epsilon/10 \cdot s_q' \geq (1-\tfrac{(l+1) \cdot \epsilon}{2}) \cdot r$
		
	\end{claim}	
	\begin{proof}
	We prove by induction on tree level. When $l=0$ ($r \leq 1$), if density of an interval $I$, $d_{c,\{I\},\kappa}(I) \geq O(\tfrac{n \log n}{\lambda^t})$, then for each color $\chi$, $\phi_\kappa^\chi(I)$ is a r.v. bounded by $1/\log n$ and expectation $\lambda^{-t}$, and since we sample $\lambda^t$ i.i.d anchors, $\sum_\chi \phi_\kappa^\chi(I)$ will concentrate around its expectation $\approx 1$ and hence we will mark such interval with $-1$ whp. %
	Consider a subtree $q$ with apriori $\hat{r} = |\RC_\kappa^{l} \cap q| =\sum_{q' \text{ is a child of }q} |\RC_\kappa^l \cap q'|$ uncolored intervals. We first observe that at most $\tfrac{\epsilon}{100} \cdot \hat{r}$ uncolored intervals are in sub-trees $q'$ with $|\RC_\kappa^l \cap q'| < \tfrac{\epsilon}{100\beta}\cdot \hat{r}$. In addition, we assume the first and last sub-trees under $q$ has at most $\tfrac{\epsilon}{100} \cdot \hat{r}$ uncolored intervals each, as otherwise we can apply the inductive hypothesis directly on their intervals, given any interval that is $O_\epsilon(\tfrac{n \cdot \log n}{\Omega_\epsilon(\hat{r})\lambda^t})$-dense is also $O_\epsilon(\tfrac{n \cdot \log n}{r \lambda^t})$-dense (which can be compounded at most $\epsilon^{-1}$ times as well), and hence the problem reduces to analyzing the rest of the intervals.
		
	For the rest of the sub-trees, we use the inductive hypothesis and Fact \ref{ft::sum_adjacent} to argue there are $(1-\tfrac{l \cdot \epsilon}{2} - \tfrac{\epsilon}{100} - \tfrac{2\epsilon}{100} - \tfrac{2\epsilon}{10}) \cdot \hat{r} = (1-\tfrac{l \cdot \epsilon}{2} - 0.23 \epsilon) \cdot \hat{r}$
	intervals in $q$ with relative density $d_{c, q, \kappa}(I) = O_\epsilon(\tfrac{n \cdot \beta \cdot \log n}{\hat{r} \cdot \lambda^t})$.
	  %
	Now, consider 3 cases when coloring level $l$. In the below, note $r \leq \hat{r}$ (ie we never uncolor an interval), and relative density of interval is monotonically decreasing as we go up the tree.%
	
	\begin{enumerate}
		\item If the number of intervals $I \in \BC_{\beta^l}(q)$ %
		with $d_{c, \BC_{\beta^l}(q), \kappa}(I) < O_\epsilon\left(\tfrac{n \log n}{\hat{r} \cdot \lambda^t}\right)$ is at least $\tfrac{10}{\epsilon} \cdot \hat{r}$, then the inductive claim holds.
		
		\item Otherwise, if the number of intervals $I \in q$ with density $d_{c, q, \kappa}(I) \in \tfrac{n}{\hat{r} \cdot \lambda^t} \cdot [O(\tfrac{\log n}{\epsilon}),\beta \log^2 n]$ is bigger than $\tfrac{\epsilon}{4} \cdot \hat{r}$, then consider an interval $I \in q \cap \RC_\kappa^l$. %
		On one hand, $\BC_{\beta^l}(I)$ contains a subset of size $\tfrac{\epsilon}{4} \cdot \hat{r}$ with density $\tfrac{n}{\hat{r} \cdot \lambda^t} \cdot [O(\tfrac{\log n}{\epsilon}),\beta \log^2 n]$, and hence with high probability, $\sum_\chi \tfrac{\phi_\kappa^\chi(I)}{100 \hat{r}/\epsilon} - \tfrac{1}{\beta \log^2 n}\geq \tfrac{\epsilon^2}{500} \cdot \hat{r}$ (using a similar argument to the base case where $l=0$).
		On the other hand, since there are at most $\tfrac{10}{\epsilon} \cdot \hat{r}$ intervals $I' \in \BC_{\beta^l}(q)$ %
		with $d_{c, \BC_{\beta^l}(q), \kappa}(I') < O_\epsilon\left(\tfrac{n \log n}{\hat{r} \cdot \lambda^t}\right)$, then we derive by inductive hypothesis:
		\begin{itemize}
			\item Let $q_1,q_2,q_3,q_4$ be the 2 leftmost and 2 rightmost sub-trees at level $l-1$ which intersects with $\BC_{\beta^l}(I)$. Then $|(q_1 \cup q_2 \cup q_3 \cup q_4) \cap \RC_\kappa^l| \leq \tfrac{20}{\epsilon} \cdot \hat{r}$. (otherwise, we would have $\tfrac{10}{\epsilon} \cdot \hat{r}$ intervals $I' \in \BC_{\beta^{l-1}}(q_1 \cup q_2 \cup q_3 \cup q_4) \subseteq \BC_{\beta^l}(q)$ with $d_{c, \BC_{\beta^l}(q), \kappa}(I') < O_\epsilon\left(\tfrac{n \log n}{\hat{r} \cdot \lambda^t}\right)$).
			\item Hence, using the above arguments on children of adjacent sub-trees within $\BC_{\beta^l}(I)$, if $|\BC_{\beta^l}(I) \cap \RC_\kappa^l| > \tfrac{100}{\epsilon} \cdot \hat{r}$, %
			then %
			we should have $(1- \tfrac{1}{2})|\BC_{\beta^l}(I) \cap \RC_\kappa^l| - \tfrac{20}{\epsilon} \cdot \hat{r} -  \tfrac{10}{\epsilon} \cdot \hat{r} = \Omega(|\BC_{\beta^l}(I) \cap \RC_\kappa^l|)$ intervals $I' \in \BC_{\beta^l}(I)$ with density $d_{c, \BC_{\beta^l}(q), \kappa}(I') \in \tfrac{n}{\hat{r} \cdot \lambda^t} \cdot [O(\tfrac{\log n}{\epsilon}),\beta \log^2 n]$ as well.
		\end{itemize}
		 %
		 Therefore, with high probability, $\sum_\chi \tfrac{\phi_\kappa^\chi(I)}{|\BC_{\beta^l}(I) \cap \RC_\kappa^l|} - \tfrac{1}{\beta \log^2 n} = \Omega(\hat{r})$.

		In either case, 
		we color $I$ whp, and therefore then the claim follows as we color all of $q$ whp. %
				
		
		\item If neither (1) nor (2) holds, then we have $(1-\tfrac{l \cdot \epsilon}{2} - 0.23 \epsilon - 0.25 \epsilon) \cdot \hat{r} < (1-\tfrac{(l+1) \cdot \epsilon}{2}) \cdot r $ intervals with relative density $d_{c, q, \kappa}(I) = \tO_\epsilon(\tfrac{n}{\hat{r} \cdot \lambda^t})$ (as $\BC_{\beta^{l-1}}(q') \subseteq q$ for any non-border sub-tree), and the claim follows.
	\end{enumerate}
	Since one of the above 3 cases above must hold, we proved the inductive assumption continues to hold at the end of level $l$ as well. This concludes the proof of the claim.
	\end{proof}
	
	Note that since each interval has density at least $1$, this proves that at the top level, $r = O_\epsilon(n/\lambda^t)$ as needed.
\end{proof}

\ns{change $n$ to $|\SC|$ once dealing with already matched intervals.}

==> newalgo-correctness.tex <==
\subsection{Correctness}

Fix an alignment $\pi: \XC \rightarrow \YC \cup \{ \bot \}$. We define the {\em extension of $\pi$}, $\widehat{\pi}: \IC \rightarrow \IC \cup \{ \bot \}$, such that,

$$\widehat{\pi}[I] = \begin{cases}
\pi[I] & I \in \XC \\
\pi^{-1}[I] & I \in \YC
\end{cases}$$

For the rest of this section, when we mention an alignment $\pi$, we loosely refer to its extension.
We also define,

\begin{definition}[Corrupted interval - new]
	Fix $w \in \N$, alignment $\pi \in \Pi$, and coloring $\kappa$. Then an interval $I \in \IC_w$ is
        a {\em $(\kappa,\pi,c)$-corrupted interval} if either
        \begin{enumerate}
       \item $\pi(I)=\bot$;
       \item $\cad(I,\pi[I]) > c$; or
        \item $I \not\equiv_\kappa \pi[I]$.
      \end{enumerate}
\end{definition}





We define the set $\EC_\kappa \subseteq \IC$ as the subset of {\em $(\kappa,\pi,c)$-corrupted intervals}.

Finally, we define a measurement $\rho_\kappa^l(I)$ to capture the ``corruptness'' of an interval ball with respect to the number of uncolored intervals as follows, $\rho_\kappa^l(I) = \tfrac{|\BC_{\beta^l}(I) \cap \EC_\kappa|}{| \BC_{\beta^l}(I) \cap \RC^{l}_\kappa|}$.

\ns{need to define in a way that $\rho_{\kappa'}^l(I) = \tfrac{|\BC_{\beta^l}(I) \cap \EC_{\kappa'}|}{| \BC_{\beta^l}(I) \cap \RC^{l}_\kappa|}$.}


Our main correctness claims follow.

First, we derive the total ``corruptness'' of uncolored intervals is proportional to the number of corrupted intervals.
\begin{lemma}\label{lm::rho_bound}
	Fix $\kappa, l, n, \RC^{l}_\kappa$. We have that $\sum_{I \in \RC^{l}_\kappa} \rho_\kappa^l(I) = O(|\EC_\kappa|)$.
\end{lemma}

\begin{proof}
	Fix a function $f = \begin{cases} 
      1 & I \in \EC_\kappa \\
      0 & I \notin \EC_\kappa
     \end{cases}$, $\SC=\RC_\kappa^l$ and $s = \beta^l$. We invoke Lemma \ref{lm::cost_fg} and obtain the claim.
     
	
	 %
	 %
\end{proof}

Next, we show that the expected $\ell1$ distance the palettes of intervals and their corresponding intervals in $\pi$ is bounded by their ``corruptness'' parameter.

\begin{lemma}\label{lm::ham_dist}
	Fix $t,c,w,l \in \N$, %
	alignment
        function $\pi \in \Pi$. Fix input coloring $\kappa'$ and remaining set $\RC^{l}_{\kappa}$ for some output coloring $\kappa$ at step $t$. Consider $I \in \RC^{l}_{\kappa}$, and fix $\rho= \rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])$.

     Then we have by expectation (over the random choice of anchors), that, 
     $$\E\left[\frac{\normo{\psi^l_{\kappa}(I) -
           \psi^l_{\kappa}(\pi[I])}}{1 + \normo{\psi^l_{\kappa}(I)} +
         \normo{\psi^l_{\kappa}(\pi[I])}}\right] = O(\rho)$$.
     

\end{lemma}

\ns{I think formally we should use $\E\left[\frac{\normo{\psi^l_{\kappa}(I) - \psi^l_{\kappa}(\pi[I])}}{1 + \normo{\psi^l_{\kappa}(I)} + \normo{\psi^l_{\kappa}(\pi[I])}}\right] = O(\rho)$}

\ns{we can also make the threshold non-deterministic, eg uniform in $[1,2]/\beta \log n$, which will probably make it easier to prove.}

\begin{proof}
Let $\gamma$ be the threshold, chosen at random from $[\gamma_0, 2\gamma_0]$.


Fix $\delta = \tfrac{\rho}{\beta^l} \cdot | (\BC_{\beta^l}(I) \cup
\BC_{\beta^l}(\pi[I])) \cap \RC^{l}_\kappa|$. Let $P=|\RC^{l}_\kappa
\cap \BC_{\beta^l}(I)|$ and
$p_\chi=\phi_{\kappa}^\chi(\BC_{\beta^l}(I))$. Similarly, let
 $Q=|\RC^{l}_\kappa
\cap \BC_{\beta^l}(\pi[I])|$, and
$q_\chi=\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))$.
Then, we can rewrite the $\ell_1$ norm as:

\begin{align*}
  \normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])}
  &=
                \sum_\chi \left| \max
                \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(I))}{|\RC^{l}_\kappa
                  \cap \BC_{\beta^l}(I)|} - \gamma,0\right\} - \max
                \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))}{|\RC^{l}_\kappa
                  \cap \BC_{\beta^l}(\pi[I])|} - \gamma,0\right\} \right| \\ 
  &=
                \sum_\chi \left| \max
                \left\{\tfrac{p_\chi}{P} - \gamma,0\right\} - \max
                \left\{\tfrac{q_\chi}{Q} - \gamma,0\right\} \right| \\ 
  &=
                \sum_\chi \left| \max
                \left\{\tfrac{p_\chi}{P} - \gamma,0\right\} - \max
                \left\{\tfrac{q_\chi}{P}-\tfrac{q_\chi}{Q}\cdot(Q/P-1) - \gamma,0\right\} \right| \\ 
\end{align*}

Wlog, we can assume that $P<Q$. We note that
$\left|P-Q\right|=\big\vert |\RC^{l}_\kappa \cap \BC_{\beta^l}(I)| -
|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|\big\vert \leq \delta
\beta^l$ since the sets $\BC_{\beta^l}(I)$ and $\BC_{\beta^l}(\pi[I])$
are not {\em $(\delta,\kappa,\pi,c)$-corrupted interval sets}. Hence,
$\tfrac{Q}{P}-1\le \tfrac{\delta \beta^l}{P}\le \rho(1+Q/P)$ (by
definition of $\delta$), and hence $Q/P-1\le O(\rho)$.
Let $\eta=Q/P-1\in[0,O(\rho)]$. We have:

\begin{align*}
  \normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])}
  &=
                \sum_\chi \left| \max
                \left\{\tfrac{p_\chi}{P} - \gamma,0\right\} - \max
                \left\{\tfrac{q_\chi}{P}-\eta\tfrac{q_\chi}{Q} - \gamma,0\right\} \right|
\end{align*}

Let $z_i=\left| \max
\left\{\tfrac{p_\chi}{P} - \gamma,0\right\} - \max
\left\{\tfrac{q_\chi}{P}-\eta\tfrac{q_\chi}{Q} -
\gamma,0\right\} \right|$. If $p_\chi/P\le \gamma$ or $q_\chi/Q\le \gamma$,
then we have that $z_i \le
\left[\psi^l_\kappa(I)\right]_\chi+\left[\psi^l_\kappa(\pi[I])\right]_\chi$ (i.e., the
value of the coordinate $\chi$). Otherwise, we have that:
$$
z_i\le p_\chi/P-\gamma-(q_\chi/P-\eta q_\chi/Q-\gamma)\le \tfrac{|p_\chi-q_\chi|}{P}+\eta\tfrac{q_\chi}{Q}=\tfrac{|p_\chi-q_\chi|}{P}+\eta\left[\psi^l_\kappa(\pi[I])\right]_\chi+\eta\gamma.
$$

\aanote{still to be finished here... doesn't quite what we want --
  there's an extra log factor...}

$$
  \normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])}
\le \sum_\chi \left| \tfrac{p_\chi}{P}-\tfrac{q_\chi}{Q}\right|
\le \sum_\chi \tfrac{\left| p_\chi-q_\chi\right|}{P}+\sum_\chi \left|
\tfrac{q_\chi}{P}-\tfrac{q_\chi}{Q}\right|
=\tfrac{1}{P}\sum_\chi \left| p_\chi-q_\chi\right|+\sum_\chi
\tfrac{q_\chi}{Q}\cdot (\tfrac{Q}{P}-1).$$


It remains to compute (the expected value of) $\sum_\chi \left|
p_\chi-q_\chi\right|$, i.e., expected difference in potential. 
Let us count the expected potential distance for any fixed color. We note that if an interval $I' \in \BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ is matched to some anchor $A$, and $I'$ is not {\em $(\kappa',\pi,c)$-corrupted interval}, then the same potential will be added to $\pi[I']$ (assuming perfect neighborhoods). Hence the potential distance can be generated from either corrupted intervals, or intervals $I' \in \BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ where $\pi[I']$ is not in the corresponding ball.
    
    Since $\BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ is not a {\em $(\delta,\kappa,\pi,c)$-corrupted
          interval set}, then there exists at most $O(\delta \beta^l)$ corrupted intervals in the balls. Furthermore, the number of ball ``mismatches'' (i.e. where $I'$ in ball, but $\pi[I']$ not in corresponding ball) is bounded by $O(\delta \beta^l)$ as well (for each interval mismatch there is a unique corrupted interval $I''$ where $\pi[I'']=\bot$).
    
    We therefore conclude that the potential distance is bounded by potential generated from a subset of $O(\delta \beta^l)$ intervals. %
    
    Since the expected potential of each interval is precisely 1, we get:
    
    \begin{align*}
    \E\left[\normo{\psi^l_\kappa(I) - \psi^l_\kappa(\pi[I])}\right]
    &\leq \tfrac{1}{P} \E\left[\sum_\chi \big\vert
      \phi_{\kappa}^\chi(\BC_{\beta^l}(I)) -
      \phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))\big\vert\right] +
    O(\rho\cdot(\|\psi^l_{\kappa}(I)\|_1+\|\psi^l_\kappa(\pi[I])\|_1)) \\
    &\leq O\left(\tfrac{\delta \beta^l}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}\right) +  O(\rho\cdot(\|\psi^l_{\kappa}(I)\|_1+\|\psi^l_\kappa(\pi[I])\|_1))	\\
    &\leq \rho \cdot O\left(1 + \normo{\psi^l_{\kappa}(I)}+ \normo{\psi^l_{\kappa}(\pi[I])}\right),
    \end{align*}
    completing the proof.


                  
\aanote{old:}
We first note that 
	\begin{align*}
		\normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])} &=
                \sum_\chi \big\vert \max
                \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(I))}{|\RC^{l}_\kappa
                  \cap \BC_{\beta^l}(I)|} - \tfrac{1}{\beta \log
                  n},0\right\} - \max
                \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))}{|\RC^{l}_\kappa
                  \cap \BC_{\beta^l}(\pi[I])|} - \tfrac{1}{\beta \log
                  n},0\right\} \big\vert \\ 
		&= \tfrac{\sum_\chi \big\vert \max
                  \left\{\phi_{\kappa}^\chi(\BC_{\beta^l}(I)) -
                  \tfrac{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}{\beta
                    \log n},0\right\} - \tfrac{|\RC^{l}_\kappa \cap
                    \BC_{\beta^l}(I)|}{|\RC^{l}_\kappa \cap
                    \BC_{\beta^l}(\pi[I])|}\max
                  \left\{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I])) -
                  \tfrac{|\RC^{l}_\kappa \cap
                    \BC_{\beta^l}(\pi[I])|}{\beta \log n},0\right\}
                  \big\vert}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}
		\end{align*}	
		
		The second quantity in the nominator can be rewritten as,
		
		$$\left(1 + \left(\tfrac{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|}-1\right)\right)\max \left\{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I])) - \tfrac{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|}{\beta \log n},0\right\}$$
	
	which simplifies to:
			$$\max \left\{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I])) - \tfrac{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|}{\beta \log n},0\right\} + \big\vert|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)| - |\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|\big\vert\max \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|} - \tfrac{1}{\beta \log n},0\right\}$$
          
          


	Now, the first quantity can be upper bounded by,
	$$\max \left\{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I])) - \tfrac{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])| + |\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|}{2\beta \log n},0\right\} + \big\vert|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)| - |\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|\big\vert \left(\max \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(I))}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|} - \tfrac{1}{\beta \log n},0\right\}\right)$$
	
	 Hence, we can upper bound $\normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])}$ with,
	$$
	\tfrac{\sum_\chi \big\vert \phi_{\kappa}^\chi(\BC_{\beta^l}(I)) - \phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))\big\vert + \big\vert|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)| - |\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|\big\vert \left(\sum_\chi \max \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(I))}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|} - \tfrac{1}{\beta \log n},0\right\} + 2\sum_\chi \max \left\{\tfrac{\phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|} - \tfrac{1}{\beta \log n},0\right\}\right)}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}
	$$
	
	\ns{check the above.}
	
	Now, since the sets $\BC_{\beta^l}(I)$ and $\BC_{\beta^l}(\pi[I])$ are not {\em $(\delta,\kappa,\pi,c)$-corrupted
          interval sets}, then $\big\vert |\RC^{l}_\kappa \cap \BC_{\beta^l}(I)| - |\RC^{l}_\kappa \cap \BC_{\beta^l}(\pi[I])|\big\vert \leq \delta \beta^l$. Hence we can upper bound the above quantity by
          
          
    	$$
	\tfrac{\sum_\chi \big\vert \phi_{\kappa}^\chi(\BC_{\beta^l}(I)) - \phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))\big\vert + \delta \cdot \beta^l \cdot \left(\normo{\psi^l_{\kappa}(I)} + 2\normo{\psi^l_{\kappa}(\pi[I])}	\right)}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}
	$$
	
	And by definition of $\rho$, we obtain
	
	\begin{equation}
	\normo{\psi^l_{\kappa}(I) - \psi^l_\kappa(\pi[I])} \leq \tfrac{\sum_\chi \big\vert \phi_{\kappa}^\chi(\BC_{\beta^l}(I)) - \phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))\big\vert}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|} + O(\rho) \cdot \left(\normo{\psi^l_{\kappa}(I)} + \normo{\psi^l_{\kappa}(\pi[I])}	\right)	
	\end{equation}

          
          \ns{check and simplify all the above!}
          
  
  	
          
    Now, let us count the expected potential distance for each color. We note that if an interval $I' \in \BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ is matched to some anchor $A$, and $I'$ is not {\em $(\kappa',\pi,c)$-corrupted interval}, then the same potential will be added to $\pi[I']$ (assuming perfect neighborhoods). Hence the potential distance can be generated from either corrupted intervals, or intervals $I' \in \BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ where $\pi[I']$ is not in the corresponding ball.
    
    Since $\BC_{\beta^l}(I) \cup \BC_{\beta^l}(\pi[I])$ is not a {\em $(\delta,\kappa,\pi,c)$-corrupted
          interval set}, then there exists at most $O(\delta \beta^l)$ corrupted intervals in the balls. Furthermore, the number of ball ``mismatches'' (i.e. where $I'$ in ball, but $\pi[I']$ not in corresponding ball) is bounded by $O(\delta \beta^l)$ as well (for each interval mismatch there is a unique corrupted interval $I''$ where $\pi[I'']=\bot$).
    
    We therefore conclude that the potential distance is bounded by potential generated from a subset of $O(\delta \beta^l)$ intervals. %
    
    Since the expected potential of each interval is precisely 1, we get:
    
    \begin{align*}
    \E\left[\normo{\psi^l_\kappa(I) - \psi^l_\kappa(\pi[I])}\right] &\leq \tfrac{ \E\left[\sum_\chi \big\vert \phi_{\kappa}^\chi(\BC_{\beta^l}(I)) - \phi_{\kappa}^\chi(\BC_{\beta^l}(\pi[I]))\big\vert\right]}{{| (\BC_{\beta^l}(I) \cap \RC^{l}_\kappa|}} + \rho \cdot \normo{\psi^l_{\kappa}(\pi[I])} \\
    &\leq O\left(\tfrac{\delta \beta^l}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|}\right) +  \rho \cdot \normo{\psi^l_{\kappa}(\pi[I])}	\\
    &\leq \rho \cdot O\left(1 + \normo{\psi^l_{\kappa}(\pi[I])}\right)
    \end{align*}


        
    as needed.
\end{proof}

As a result, we can bound the corruption growth each level.

\begin{lemma}\label{lm::corruption_growth}
	Fix $t,c,w \in \N$, $\eps, \delta \in [0,1]$, alignment
        function $\pi \in \Pi$. Fix level $l$ with input coloring $\kappa'$ and output coloring $\kappa$.%
        Let $k=|\EC_{\kappa'} \cup \EC_{\kappa}|$ be the number of expensive interval at level $l$.
          Then, \textsc{ColorIntervals} at level $l$ colors $\kappa$ such that at the next level we have that $|\EC_{\kappa'} \cup \EC_{\kappa}| = O(\tfrac{k}{\epsilon^2 \cdot \eta})$ %
         with probability $1-\eta$.
\end{lemma}

The proof is provided in the next section.

Finally, we derive,

\begin{lemma}\label{lm::existence_good_color}
	Fix $t,c,w \in \N$, $\eps$, alignment
        function $\pi \in \Pi$. Suppose we call to \textsc{MatchIntervals} at step $t$ with coloring $\kappa$. %
          Then with high probability, we generate  a coloring $\kappa' \in \Kappa$ where $|\EC_{\kappa'}| = O(\epsilon)^{-3/\epsilon} \cdot |\EC_{\kappa}|$.        %
\end{lemma}
\begin{proof}
	Fix a coloring $\kappa_j$. From Lemma \ref{lm::corruption_growth}, at each level $l \in [\log_\beta n]$ we have $O(\epsilon^{-3})$ factor growth in corruption with probability $1-\epsilon/2$, and by the union bound we get overall blow-up $O(\epsilon)^{-3/\epsilon}$ with probability $1/2$ (as we have $1/\epsilon$ levels). Since generate $O(\log n)$ i.i.d colorings, the claim follows.
\end{proof}

\ns{Actually, I think we don't need union bound / markov as the corruption growth r.v. are independent, hence we can show the expectation of product is product of expectations, and we save some factor in exponent.}


\subsection{Proof of Lemma \ref{lm::corruption_growth}}
\begin{proof}[Proof of Lemma \ref{lm::corruption_growth}]



Fix level $l$, and consider an {\em uncorrupted interval} $I \in \RC^{l}_\kappa \setminus \EC_\kappa \setminus \EC_{\kappa'}$. We show that the probability to {\em corrupt} $I$ is bounded by $O(\rho/\epsilon^2)$, where $\rho = \rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])$. Note that if $\rho \geq \tfrac{\epsilon^2}{100}$ the statement is trivial, so we assume $\rho < \tfrac{\epsilon^2}{100}$. We also invoke Lemma \ref{lm::ham_dist}, and get that $\E\left[\tfrac{\normo{\psi^l_\kappa(I) - \psi^l_\kappa(\pi[I])}}{1 + \normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])}}\right] = O(\rho)$. 

	Note that the only way to corrupt $I$ at level $l$ is by having $I$ and $\pi[I]$ contain different colors at the end of level $l$, which can happen in one of two ways.
	
	\paragraph{Threshold separation.} Here we bound the probability that precisely one of $\psi^l_\kappa(I), \psi^l_\kappa(\pi[I])$ pass the threshold test and will be colored while the other one remain uncolored. 
	
	First, we observe that if $\normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])} > 1$, both will pass the test unless $\left| \normo{\psi_\kappa^l(I)} - \normo{\psi_\kappa^l(\pi[I])}\right| > \normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])}-O(\epsilon^2)$. The LHS is upper bounded by $\normo{\psi_\kappa^l(I)-\psi_\kappa^l(\pi[I])}$ and the RHS is $\Omega(1 + \normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])})$. Hence the inequality can happen with probability $1-O(\rho)$ (by Markov).
	 Otherwise, we condition on $\normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])} \leq 1$ and hence $E[\normo{\psi_\kappa^l(I)} - \normo{\psi_\kappa^l(\pi[I])}] = O(\rho)$. Since the probability $T$ will be sampled within the range is at most $\left(\normo{\psi_\kappa^l(I)} - \normo{\psi_\kappa^l(\pi[I])}\right) \cdot O(\tfrac{1}{\epsilon^{2}})$ (which happens if the entire $\ell1$ range falls within the threshold sampling range), then the overall separation probability is bounded by $O(\tfrac{\rho}{\epsilon^2})$.
	 
	 \paragraph{WMH not colliding.} If both pass the threshold test, then we have that $\normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])} = \Omega(\epsilon^2)$. We now apply Theorem \ref{?} and obtain collision probability $1-\tfrac{\normo{\psi_\kappa^l(I) - \psi_\kappa^l(\pi[I])}}{\normo{\psi_\kappa^l(I)} + \normo{\psi_\kappa^l(\pi[I])}}$ which (by expectation) is $1-O(\tfrac{\rho}{\epsilon^2})$.

	By the union bound over the above 2 failure probabilities, we get overall probability of corruption $O(\tfrac{\rho}{\epsilon^2})$ as well.
	
	Second, summing over all $I \in \RC_\kappa^l$, we use Lemma \ref{lm::rho_bound} to bound the expected number of newly corrupted intervals.
	$$\E [\text{newly corrupted intervals}] = \sum_{I \in \RC^{l}_\kappa} \Pr[\text{corrupt } I] = \sum_{I \in \RC^{l}_\kappa} O(\tfrac{\rho_\kappa^l(I) + \rho_\kappa^l(\pi[I]) + \rho_{\kappa'}^l(I) + \rho_{\kappa'}^l(\pi[I])}{\epsilon^2}) = O(\tfrac{|\EC_\kappa \cup \EC_{\kappa'}|}{\epsilon^2}).$$
	
	
	The soundness of the Lemma follows the Markov inequality.
\end{proof}


\subsection{old stuff}

For sets of intervals, we define the following.

\begin{definition}[Corrupted set of intervals - new]
	Fix $c, w \in \N$, $\delta \in [0,1]$, alignment
        $\pi \in \Pi$, and coloring $\kappa$. Then an interval set $\SC
        \subseteq \IC_w$ is {\em
          $(\delta,\kappa,\pi,c)$-corrupted} if there exists a
        subset $\SC_\delta \subseteq \SC$ of size $\delta \cdot
        |\SC|$ such that for each $I \in \SC_\delta$, we have that $I$ is {\em $(\kappa,\pi,c)$-corrupted interval}.
\end{definition}


We define the set $\EC_\kappa \subseteq \IC$ as the subset of {\em $(\kappa,\pi,c)$-corrupted intervals}.

Finally, we define a measurement $\rho_\kappa^l(I)$ to capture the ``corruptness'' of an interval ball with respect to the number of uncolored intervals as follows, $\rho_\kappa^l(I) = \max_\delta(\delta \cdot \tfrac{\beta^l}{| \BC_{\beta^l}(I) \cap \RC^{l}_\kappa|}) \text{ s.t. } \BC_{\beta^l}(I)$  is a {\em $(\delta,\kappa,\pi,c)$-corrupted interval set}.




==> newalgo.tex <==
\section{New algo}

\subsection{Algo overview}
As previously, our algorithm consists of 2 main subroutines: matching phase and coloring phase.
The matching phase is now recursive, but works in a similar fashion. First, we sample $\lambda^t$ anchors. Then, we match those anchors with all intervals in its partition, add relevant edges, and assign potential scores. The matching phase is simpler now as we only have a single ``input'' coloring $\kappa$, and produces an ``output'' coloring  $\kappa'$ which is ``good'' with constant probability. To obtain a ``good'' coloring with high probability, we produce $O(\log n)$ such colorings and  recourse on each one.

In the coloring phase, we generate %
a coloring based on potential scores by hashing intervals into colors as will be described below. The coloring phase works in {\em levels} $l \in \log_\beta n$. Levels correspond to ball radiuses $\beta^l$ around each intervals where we look for matches. At each level, we color a subset of intervals and leave the remaining ``uncolored'' (as will be defined).%
\subsection{Definitions}

\paragraph{Coloring.} A coloring $\kappa: \IC \rightarrow \nu \cup \{-1,0\}$ is a mapping from intervals to colors $\chi \in \nu \cup \{-1,0\}$. We refer to $0$ as the empty color, and intervals where $\kappa(I)=0$ as {\em uncolored intervals}. Intervals with $\kappa(I)=-1$ are {\em already matched}, meaning we do no longer need to match such intervals, and hence such intervals will be disregarded in future steps.

The mapping above defines an equivalence relation $\equiv_\kappa$ such that $I_1 \equiv_\kappa I_2$ iff 2 intervals shares a color in $\kappa$, and a partitioning of intervals for equivalence groups based on their color in $\kappa$. We define $\PC_\kappa(I)$ as the projection of $I$ into its partition. 

A coloring set $\Kappa$ is a set of coloring as defined above.



\paragraph{Potential scores.}
We use potential scores $\phi$s as previously. Since we assume perfect neighborhoods, then the expected potential of each interval is precisely $1$, and the expected $\ell1$ distance between the $\phi$ vectors of $\beta^l$-size balls around corresponding $x$ and $y$ intervals is bounded by the number of {\em corrupted} intervals in such balls (to be defined). As we look to color intervals based on potential scores, we look to convert the $\phi$ scores of balls into $\psi$ scores that are, (1) sparse (to allow for max intervals per color), and (2) have a bounded Jaccard distance, to allow for soundness of our coloring procedure.

We define $\psi^l_\kappa(I) \in \R^{\lambda^t}$ as a (sparse) color vector, each coordinate is as follows:

$$(\psi^l_\kappa(I))_\chi = \max \left(\frac{\phi_{\kappa}^\chi(\BC_{\beta^l}(I))}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|} - \tfrac{1}{\beta \log^2 n},0\right)$$



where $\RC^{l}_\kappa$ is the set of {\em uncolored intervals} at level $l$.%
We sometimes refer to $\psi^l_\kappa(I)$ as the {\em palette} of $I$.

\subsection{Thresholds, Jaccard Similarity and WMH sampling}

Each interval which we color at some level $l$ will get be colored using a unique weighted minhash (WMH) function. We will use the following bound on the collision probability of WMH sampling, showing the success probability is proportional to the Jaccard similarity between the {\em palettes} of $I$ and $\pi[I]$ for each $I \in \IC$.

\ns{Add and cite Theorem}

One can observe that since the $\phi$ $\ell1$ distance is, by expectation, at most the number of corrupted intervals in ball, then the $\psi$ $\ell1$ distance is, by expectation, $O(\tfrac{|\EC \cap \BC_{\beta^l}(I)|}{|\RC^{l}_\kappa \cap \BC_{\beta^l}(I)|})$, where $\EC$ is the set of already corrupted intervals (to be defined).
To ensure the Jaccard distance is bounded as well, we define a minimum threshold norm for the $\psi^l_\kappa(I)$. We will use weighted minhash sampling from the palettes of intervals which pass the threshold test in order to obtain colors that disagree with probability proportional to the Jaccard distance, hence we can bound the corruption rate at each level as well. Note that we do not necessarily manage to color all intervals per coloring, and intervals that do not pass the threshold test will remain {\em uncolored} for the next {\em level}. Nevertheless, we show that with high probability, only a few number of intervals do not pass the threshold test at any level and remained {\em uncolored} when we are done, hence we guarantee {\em uncolored} partition size is similarly bounded. The threshold test will be random, to avoid a ``border'' issue. 

Overall, we show that since we have constant number of levels, then the corruption rate is only a function of $\epsilon$, and since we only have constant number of steps then the total corruption growth is only a function of $\epsilon$ as well.







\subsection{Algorithm}
In the below, parameters are as in previous sections, except now we have $\beta = \lambda = n^\epsilon$ (rather than $n^{\epsilon^2}$).
\begin{algorithm}[H]
\caption{Matching Phase - Color Intervals}
\begin{algorithmic}[1]
\label{alg::matching.color_new}
\Function{ColorIntervals}{$\RC^l_\kappa,\kappa,l$}
\State Sample $T%
\sim \epsilon^2  \cdot [\tfrac{1}{100},\tfrac{1}{50}]$ uniformly.
\State Sample  %
 WMH function $h$.
\State Compute all
$\psi^l_\kappa(I)$ for 
$I \in \RC^{l}_\kappa$ as above.
\Comment by adjusting 2 coordinates each time


      	\For {$I \in \RC^{l}_\kappa$}
    		\If {$\normo{\psi^l_\kappa(I)} \geq T$}
    		\State  $\kappa(I) \gets \begin{cases} 
      -1 & l=0 \\
      h(\psi^l_\kappa(I)) & l>0
   \end{cases}$
      		 %
          \EndIf
        \EndFor
        \State \Return $\kappa$.
\EndFunction	
\end{algorithmic}
\end{algorithm}

\ns{for leaves $l=0$, assign color $-1$ and remove from $\SC$ for future steps in each coloring.}

\ns{improve notation.}

In the below, we make an initial call with:
\begin{enumerate}
	\item $t \gets 1 .\SC \gets \IC$.
	\item $\forall I\in \IC, \kappa(I) \gets 0$.
\end{enumerate}

\begin{algorithm}[H]
\caption{Matching Phase - New}
\begin{algorithmic}[1]
\label{alg::matching.new}	

\Function{MatchIntervals}{$\SC, \GC_w, c, \kappa,t$}
				\State Initialize $\Kappa = \{\kappa_1,\ldots,\kappa_m\}$.
				
				\State $G \gets$ unweighted and undirected graph with nodes $I \in \IC$ and no edges. 

				 
				\For {$j \in [m]$}  
				\For {$l \in 0\ldots \log_\beta n$}
					\State $\phi_{\kappa_j} \gets \vec{0}$.%

					\For {$\chi \in [\lambda^t]
                                  $}
				\State Sample $A%
				\sim \SC$ uniformly at random.%
				\State $\A%
				\gets $ \textsc{ClusterAnchor}($A,\PC_{\kappa}(A), \GC_w, c$).
				\State Add edges $(A,I)$ for $I \in \A$ to $G$.
				\State $\textsc{AssignPotential}(\A,A,\chi,\GC_w, c)$.
				\EndFor
						\State $\RC^{l}_{\kappa_j} \gets \{I \in \SC \mid \kappa_j(I) = 0\}$.
						\State $\kappa_j \gets \textsc{ColorIntervals}(\RC^{l}_{\kappa_j},\kappa_j,l)$.
				\EndFor
				\State $\SC_j \gets \{I \in \SC \mid \kappa_j(I) \neq -1\}$.
			\EndFor
		\State $G \gets \cup_{j 
		\in [m], \SC_j \neq \emptyset} \textsc{MatchIntervals}(\SC_j, \GC_w, c, \kappa_j,t+1)$.
		
	\State \Return $G$.
\EndFunction

\end{algorithmic}
\end{algorithm}


\input{newalgo-complexity}
\input{newalgo-correctness}

\input{matching}
\input{matching-complexity}
\input{matching-correctness}

\input{imperfect-N}



==> notation-table.tex <==
\begin{table}[h!]
\caption{Summary of main notations and definitions}
  \label{tab:notation}
 \centering
  \begin{tabular}{|l|l|}
    \hline
    $\nu$ & $[\lambda^t]\cup \{\un, \bot\}$ color set
    \\
    \hline
    $\mu_\kappa(I,\chi)$ & mass of $(I,\chi)$ in
    $\kappa$. $\mu_\kappa(I,*)$ is a probability distribution.
    \\
    \hline
    $E_\basec, c_i$ & $c_i= \tfrac{2\basec}{\alpha} \cdot 3^i$ and
    $E_\basec=\{c_1,\ldots c_{1/\eta}\}$, for a small constant $\eta$, dependent on
    $\epsilon$ only.
    \\
    \hline
    bad costs & For $(A,\chi')$, all $c_i$'s such that
    $\den_{\kappa'}(A,\chi')_{c_{i-1}}<
    n^\alpha \cdot \den_{\kappa'}(A,\chi')_{c_{i+1}}$. at most $O(1/\alpha)$.
    \\
    \hline
    $\phi_\kappa(I,\chi)$ & $=\mu_{\kappa'}(I,\chi')\tfrac{n}{\lambda^t}\sum_{j=0}^{j_{\max}} n^{-\alpha j}\tfrac{1}{\max\{d_{I,j},d_m\}}$ basic potential added to $(I,\chi')$ from anchor matching.
    \\
    \hline
    $\Lambda_\kappa^\zeta(I)$ & smallest interval ball containing
    $\zeta$ of $\ell_1$-mass of \un-color in $\mu$ on the left and right of $I$
    \\
    \hline
    $Z_l$ & $2^{E} \cdot \beta^l$, where $E = \{0 \ldots \lceil \log_2 n \rceil\}$.
    \\
    \hline
    $\varphi_\kappa^\zeta(I,*_{\neq \un})$ & $=T^\cc\left(\mu_\kappa(I,\un)\cdot
    \tfrac{\beta^{2l}}{\zeta^2}\cdot
    \tfrac{\phi_\kappa(\Lambda_\kappa^\zeta(I),*)}{\beta^l}\right)$
    \\
    \hline
    $T^\cc$ & $=T^{\Theta(1/\epsilon)}_{1/\beta, 1/\beta^3}$
    \\
    \hline
    $T^q_{\delta,\gamma}(x)$ & = $\begin{cases}
	x_i	&	x_i \geq \gamma \\
	0	& x_i < \delta \gamma \\
	\gamma \cdot (\tfrac{x_i}{\gamma})^q	&	\text{Otherwise}
\end{cases}$
    \\
    \hline
    $\mu_{\hat \kappa}(I,*)$ & $=\mu_\kappa(I, *_{\neq \un}) +
    \mu_\kappa(I,\un)\cdot \normalizedEllOne{\mu_\kappa(I,*_{\neq
        \un})+\sum_{\zeta\in Z_l} \varphi_\kappa^\zeta(I,*)}$ (always a
    distribution over $\chi$'s)
    \\
    \hline
    $\den_\kappa(I,\chi,\SC)$ & $= 
    \mu_\kappa(\NC_*(I) \cap \SC,\chi)$ is a vector of densities per
    cost in $E_\basec$
    \\
    \hline
    $\relden_\kappa(I,\chi,\SC)$ & $= \den_\kappa(I,\chi, \IC) \oslash \den_\kappa(I,\chi,\SC)$
    is a vector obtained by coordinate-wise division
    \\
    \hline
    $\VC$ & subsampling $\IC \times
\nu \setminus \{ \bot \}$ with prob. $\mu_{\kappa'}(V,\chi')\cdot \tfrac{k}{\beta^l}$
independently for each $(V, \chi')$
    \\
    \hline
    $\sigma_{V,\chi'}$ &  $= 
    Q_l(T^\theta\left(\Gamma_{l,\zeta}(V,\chi')\right))$
    \\
    \hline
    $\Gamma_{l,\zeta}(V,\chi')$ & a vector of costs in $E_\basec$ with
 $\Gamma_{l,\zeta}(V,\chi') =
\min\left\{\reallywidehat{\relden_{\kappa'}(V,\chi',\Lambda_\kappa^{\zeta}(V))}^{-1}\cdot
\frac{\totalmu \cdot n^{3\alpha}}{ \beta^l \cdot \lambda^t}, 1\right\}$
    \\
    \hline
$\theta_\kappa^{\zeta}(V,\chi')$ & $= 
m_\VC((V,\chi')) \cdot \begin{cases}
	\sigma_{V,\chi'}	&	\mu_{\kappa'}(\Lambda_{\kappa'}^\zeta(V),\chi') \leq \lambda \cdot \beta^6 \cdot \beta^l	\\
	1	&	\text{Otherwise}
\end{cases}$
\\
\hline
$m_\VC((V,\chi'))$ & multiplicity of $(V,\chi')$ in $\VC$
\\
\hline
$T^\theta$ & $ = T^{O(1/\epsilon)}_{\beta^{-1},1}$
    \\
    \hline

$Q_{\delta,s,F}(x)$ & $= \max_{J \subseteq [d]} a_{|J|} \cdot \min_{j
      \in J} x_j$, where $a_i = \begin{cases}
        1       & i \geq s\cdot d \\
        0       & i < (s-\delta)d \\
        1/F^{sd-i}        &       \text{Otherwise.}
\end{cases}$
    \\
    \hline
    $Q_l(x)$ & $=
    Q_{\tfrac{\epsilon}{4},1-\tfrac{l\epsilon}{2},n^{\alpha^2}}(x)$,
    where $\alpha$ is a small const
    \\
    \hline

    $\varphi_\kappa^\zeta(I,\un)$ & $= T^\un\left(\frac{\beta^{2l}}{\zeta^2} \cdot \mu_\kappa(I,\un) \cdot \min\left\{\frac{1}{k} \cdot \sum_{\chi'\in \nu \setminus \{\bot \}}\theta_\kappa^{\zeta}(\Lambda_\kappa^{\zeta}(I),\chi'),1\right\}\right)$ 
    \\
    \hline
    $T^\un$ & $=T^{O(1/\eps)}_{1/\beta, \Omega_\eps(1)}$
    \\
    \hline
    $\varphi_\kappa^0(I,\bot)$ & $= T^\cc\left(\mu_\kappa(I,\un) \cdot
\phi_{\kappa}(I, \nu \setminus \{\un, \bot
\})\right)$
\\
\hline
$\varphi_\kappa^0(I,\un)$ & $= T^\un\left(\mu_\kappa(I,\un) \cdot \tfrac{\theta_\kappa^{0}(I,\nu \setminus \{ \bot \})}{k} \right)$
\\
\hline
    $\xi_F^{\kappa}(I)$ & \pbox{20cm}{\vspace{1mm}$=1$ if $\pi[I]=\bot$
  or $\cad(I,\pi[I])>\basec$\\
  $=\dd_F(\mu_\kappa(I,*_{\neq \bot}),\mu_\kappa(\pi(I),*_{\neq \bot})) + \mu_\kappa(I,\bot) \cdot \1[\text{dist}_G(I,\pi[I])>2]$ otherwise
    }
    \\
    \hline
  \end{tabular}
\end{table}



==> prob-part.tex <==

\subsection{Proof of Lemma \ref{lm::prob_part}: probability of
  choosing a good coloring}\label{sec::prob_part}

We first show the following claim on the parameter $d_v$ of matched
interval, which will be used to bound their potential in the proof.

\begin{claim}\label{cl::potential_density}
  Consider a call to \textsc{AssignPotential}, for an anchor cluster $\A$ generated by anchor $A$, and an interval set
         $\PC_x=\PC_{\kappa_j^t}(A) \cap \XC$. For any $v\in \A$, we have $d_v
        \geq 0.9 |\NC_{c_A}(v) \cap \PC_x|$ whp.
\end{claim}

\begin{proof}
We consider two cases.	If $|\NC_{c_A}(v) \cap \PC_x| \leq |\NC_{c_A}(A) \cap \PC_x|$, then we have: $d_v \geq |\A \cap \XC| = |\NC_{c_A}(A) \cap \PC_x| \geq |\NC_{c_A}(v) \cap \PC_x|$.
	
	On the other hand, consider $|\NC_{c_A}(v) \cap \PC_x| >
        |\NC_{c_A}(A) \cap \PC_x|$, then, when we call the procedure
        {\sc ApproxDensity}, we have $\alpha=1/|\A\cap \XC|$ and hence
        $\alpha\zeta |\NC_{c_A}(v) \cap \PC_x|\ge \alpha\zeta|\A \cap
        \XC|= \zeta=\Theta(\log n)$. Thus, by standard Chernoff bound,
        the procedure will find $\ge 0.9 \alpha\zeta \cdot
        |\NC_{c_A}(v) \cap \PC_x|=\Omega(\log n)$ matches, hence $d_v
        \geq 0.9 \zeta \cdot |\NC_{c_A}(v) \cap \PC_x| / \zeta = 0.9
        |\NC_{c_A}(v) \cap \PC_x|$ as needed.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lm::prob_part}]
 We prove that, if (a) doesn't hold, then (b) must hold. To analyze
  (b), we partition possible colors $\chi$ into two classes: ``good''
  and ``bad''. We show that if $\chi$ is ``good'', then the event
  inside $\Pr[\cdot]$ holds. We then show that the probability of
  choosing a ``bad'' $\chi$ is bounded as desired. 

  We first define ``cheap'' and ``expensive'' leafs of $q_x$, loosely
  related to good/bad colors. For each
  coloring $\kappa_j^{t}$ where $j\in[m]$, we denote by $\CC_{\kappa_{j}^t}$ set of
  leafs $v \in q_x$ that are cheap and $\kappa$ is a $(v,\pi)$-good
  coloring; furthermore $\EC_{\kappa_{j}^t}$ is defined to be the rest:
	\begin{align*}
			\CC_{\kappa_{j}^t} &= \{ v \text{ is leaf of } q_x \mid \cad_w(v,\pi[v]) \leq c  \text{ and } \pi[v] \in \PC_{\kappa_{j}^t}(v) \} \\
	\EC_{\kappa_{j}^t} &= q_x \setminus \CC_{\kappa_{j}^t}
	\end{align*}
		
	Note that $\CC_{\kappa_{j}^t}$ and $\EC_{\kappa_{j}^t}$ are disjoint and contain all
        the leafs of $q_x$.
	
	
	 %
	 %
	 
	          Fix $j$ such that $q_x$ is $j$-dense (there must
                  exist such as $q_x$ is dense). Hence $
                  \psi_{\RC_x,j}(q_x) \geq \psi_{j}(q_x)
                  \geq \eps^2 \cdot k$. This means we sampled a set
                  of colors $\QC_j = \QC_{\XC,j} \cap
                  \QC_{\RC_x,j}$ where for each $\chi \in
                  \QC_{j}$, we have that $\phi_j^{\chi}(q_x) \geq
                  |q_x|/\beta$.

         

          
         
         
	
		\paragraph{Good Colors.} 
			  Fix a color $\chi \in \QC_j$, and hence with
                          $\phi_j^\chi(q_x) \ge \tfrac{|q_x|}{\beta \log n}$. A
                          ``good'' color $\chi$ is one where at
                          least 10\% of the potential
                          $\phi_j^\chi(q_x)$ originates from leafs
                          belonging to $\CC_{\kappa_{j}^t}$.
			  
			  
	Now, consider the smallest enclosing interval ball of the set
        $\{ \pi[v]\mid v \in q_x \}$ in $\HC$, denoted $B_{q_x,\pi}$. 
	 Consider any anchor $A$, and let $c_A$ be the corresponding value defined by the minimum fraction in $\textsc{ClusterAnchor}$.
 For any $X \in
         \PC_{\kappa_j^t}(A) \cap \CC_{\kappa_{j}^t} $, we have $\pi[X] \in
         \NC_{c_A + c}(A) \cap \PC_{\kappa_j^t}(A)$ --- by definition of
         $\CC_{\kappa_{j}^t}$, noting $\PC_{\kappa_j^t}(A) =
         \PC_{\kappa_j^t}(X)$ for all $X \in \PC_{\kappa_j^t}(A)$. Hence
         $|\NC_{c_A+c}(A) \cap B_{q_x,\pi} \cap
         \PC_{\kappa_j^t}(A)| \geq |\NC_{c_A}(A) \cap
         \CC_{\kappa_{j}^t} \cap \PC_{\kappa_j^t}(A)|$.

	 
	 	Since we assume (a) doesn't hold, we have that $(\max
                B_{q_x,\pi}-\min B_{q_x,\pi}) \le 2|q_x|$.  Hence, we can find 3 consecutive $q_y^1,q_y^2,q_y^3$, on same tree level as $q_x$ with $\BC_{q_x,\pi} \subseteq q_y^1 \cup q_y^2 \cup q_y^3$, hence $\phi_j^{\chi}(q^1_y) + \phi_j^{\chi}(q^2_y) + \phi_j^{\chi}(q^3_y) \geq \phi_j^{\chi}(q_x)/10$ as well (noting we always assign maximum potentials to $y$ matches). 
	 Therefore, for one of $q_y^1, q_y^2, q_y^3$ (say, w.l.o.g $q_y^1$), we have %
	 that $\phi_j^{\chi}(q^1_y) \geq %
	  \phi_j^{\chi}(q_x)/30 \geq \tfrac{|q_x|}{30\beta \log n} \geq \tfrac{|q^1_y|}{30 \beta \log n}$. 
	 
	 Since we add $\chi$ to the color-set of
         $\BC_{2|q^1_y|/w}(q^1_y)$ for all $j' \in [m]$, we also have
         $\chi \in \kappa_{j'}^{t+1}(Y)$ for all $Y \in
         \BC_{q_x,\pi}$. Hence, if $\chi$ is chosen from the
         distribution $p$ and added to coloring $\kappa_{j'}^{t+1}$,
         then $\kappa_{j'}^{t+1}$ is a $(v,\pi)$-good coloring for all
         $v\in q_x\cap \widehat {\RC_x}$.
            
	 %
		
		
	\paragraph{Bad Colors.} 
	 %
	  %
        A color
        $\chi \in \QC_j$ is ``bad'' if 90\% of the potential
        originates from leafs in $\EC_{\kappa_{j}^t}$.
        We define the random
        variable $\psi^\EC_{\RC_x,j}$ of the total
        contribution to $\psi_{\RC_x,j}$ of ``bad'' colors
        $\chi$.
	  We first decompose $\RC_x$ based on distance $c_A$ as follows:  
	  $$\RC^{c^*}_x = \{A \in \RC_x | c^* = c_A \}$$
	
     
        

        
        For a random anchor $A$, its contribution to
        $\psi_{\RC_x,j}^{\EC}(q_x)$ is at most:
        
     $$
\psi^1_{\RC_x,j}\le \min\left\{\frac{|\RC_x|}{|q_x \cap
          \RC_x| n} \cdot
\phi_{\RC_x,j}^\chi(q_x),1\right\}     \le \min\left\{\frac{|\RC_x|}{|q_x \cap
          \RC_x| n} \cdot\frac{1}{ 0.9 }\sum_{X \in
  \EC_{\kappa_{j}^t}} \frac{\1[X \in \NC_{c_A}^\XC(A) \cap
    \PC_{\kappa_{j}^{t}}(A)]\cdot  n}{d_X \lambda^t},1\right\}
$$
Using Claim \ref{cl::potential_density} on $d_X$:
$$
\psi^1_{\RC_x,j}
\le
           \min\left\{ \frac{|\RC_x|}{0.9\cdot |q_x \cap
          \RC_x|\cdot \lambda^t} \cdot\sum_{X \in \EC_{\kappa_{j}^t}} \frac{
         \1[A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]}{0.9
             \cdot |\NC_{c_A}^\XC(X) \cap \PC_{\kappa_j^t}(X)|},1\right\}
           $$

        
Overall $\psi^\EC_{\RC_x,j}$ is a sum of $k\lambda^t$ iid
copies of the random variable $\psi^1_{\RC_x,j}\in[0,1]$
(where randomness is over the choice of random anchor $A$).  To show
concentration of $\psi^\EC_{\RC_x,j}$, we first upper bound
the expectation of $\psi^1_{\RC_x,j}$. We note that, for a
corrupted interval $X \in \EC_{\kappa_{j}^t}$, the probability that
$A\in \NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)$ when $A \sim
\RC^{c^*}_x$ is:
     $$\Pr_{A
          \sim \RC^{c^*}_x}[A \in \NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]%
        = \tfrac{|\RC^{c^*}_x \cap \NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}{|\RC^{c^*}_x|}.$$

        Hence we can bound:
        
                 

	
		 
	\begin{align*}
          \E[\psi^1_{\RC_x,j}] &\leq \E_{A \sim \RC_x}
          \left[
           \frac{1.3\cdot |\RC_x|}{|q_x \cap
          \RC_x|\cdot \lambda^t} \cdot\sum_{X \in \EC_{\kappa_{j}^t}} \frac{
         \1[A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]}{|\NC_{c_A}^\XC(X) \cap \PC_{\kappa_j^t}(X)|}
        \right] \\
	&= \frac{1.3 \cdot |\RC_x|}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot \sum_{X \in \EC_{\kappa_{j}^t}}
       \E_{A \sim \RC_x} \left[\frac{\1[A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]}{|\NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}\right] \\
    &= \frac{1.3 \cdot |\RC_x|}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot  \sum_{X \in \EC_{\kappa_{j}^t}} \sum_{c^* \in c\cdot[1/\eps^2]}
       \frac{|\RC^{c^*}_x|}{
          |\RC_x|} \cdot \E_{A \sim \RC^{c^*}_x} \left[\frac{\1[A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]}{|\NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}\right] \\
        &= \frac{1.3}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot  \sum_{X \in \EC_{\kappa_{j}^t}} \sum_{c^* \in c\cdot[1/\eps^2]}
     \frac{  \E_{A \sim \RC^{c^*}_x} \left[\1[A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)]\right]\cdot |\RC^{c^*}_x|}{|\NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}  \\
	&= \frac{1.3}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot \sum_{X \in \EC_{\kappa_{j}^t}}\sum_{c^* \in c\cdot[1/\eps^2]}
        \frac{\Pr_{A \sim \RC^{c^*}_x} [A \in \NC_{c_A}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)] \cdot |\RC^{c^*}_x|}{|\NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|} \\
	&= \frac{1.3}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot  \sum_{X \in \EC_{\kappa_{j}^t}}\sum_{c^* \in c\cdot[1/\eps^2]}
        \frac{|\RC^{c^*}_x \cap \NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}{|\RC^{c^*}_x|} \cdot \frac{|\RC^{c^*}_x|}{|\NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|} \\
   	&= \frac{1.3}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot  \sum_{X \in \EC_{\kappa_{j}^t}}\sum_{c^* \in c\cdot[1/\eps^2]}
        \frac{|\RC^{c^*}_x \cap \NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|}{|\NC_{c^*}^\XC(X) \cap \PC_{\kappa_{j}^{t}}(X)|} \\
	&\leq \frac{1.3}{
          |q_x \cap  \RC_x|} \cdot \frac{1}{\lambda^t} \cdot  \sum_{X \in \EC_{\kappa_{j}^t}}
         1/\epsilon^2 \\
	&\leq \frac{1.3\cdot |\EC_{\kappa_{j}^t}|}{ |q_x \cap
           \RC_x|\cdot \epsilon^2\cdot \lambda^t}
\end{align*}

Now, since $\psi^\EC_{\RC_x,j}$ is a sum of $k \cdot
\lambda^t$ i.i.d r.v., taking values in $[0,1]$ with expectation at
most $\tfrac{1.3|\EC_{\kappa_{j}^t}|}{ |q_x \cap \RC_x|}
\cdot \tfrac{1}{\lambda^t \epsilon^2}$, we have by Bernstein inequality that
$\psi^\EC_{\RC_x,j} \leq \max\{1.5 \cdot
\E[\psi^\EC_{\RC_x,j}],O(\log n)\}\leq
\max\{\tfrac{2|\EC_{\kappa_{j}^t}|}{ |q_x \cap \RC_x|} \cdot
\tfrac{1}{\lambda^t \epsilon^2} \cdot k \cdot \lambda^t,O(\log n)\} =
\max\{\tfrac{2|\EC_{\kappa_{j}^t}|}{ |q_x \cap \RC_x| \eps^2} \cdot
k ,O(\log n)\} \leq \left(\tfrac{2|\EC_{\kappa_{j}^t}|}{ |q_x \cap
  \RC_x| \epsilon^2} + O(\tfrac{\log n}{k})\right)\cdot k$ with high
probability.



				 
		\paragraph{Bounding the overall probability in (b).} 
		With the above, we can finally show a good bound on
                $$\Pr_{\chi \sim p}
		\left[v \between_{\kappa_j^{t+1}} \pi[v] \text{ for each
                  } v \in q_x\cap \RC_x \right].$$
		
We have shown that for ``good colors'',
the above holds whp, and hence it remains to upper bound the
probability of sampling a ``bad color'' from $p$. From the definition of
distribution $p$, this sums up to,
		\begin{equation}\label{eq::prob_fail}
		\frac{\sum_{j \in [m]: q_x \text{ is } j\text{-dense}} \psi^\EC_{\RC_x,j}(q_x)}{\sum_{j \in [m]: q_x \text{ is } j\text{-dense}} \psi_{\RC_x,j}(q_x)}			
		\end{equation}

		Since $q_x\cap \RC_x$ is not
                $(\delta,\eta,\Kappa^t,\pi,c)$-corrupted, we have that
                $\Pr_{\substack{j \in [m] \\ X \in q_x \cap
                    \RC_x}} [X \in \EC_{\kappa_{j}^t}] \leq
                \delta + \eta$. Hence we can upper bound the
                numerator:
 		
		$$\sum_{j \in [m]: q_x \text{ is } j\text{-dense}} \psi^\EC_{\RC_x,j}(q_x) \leq \sum_{j \in [m]} \psi^\EC_{\RC_x,j}(q_x) \leq \sum_{j \in [m]}  \left(\tfrac{2|\EC_{\kappa_{j}^t}|}{ |q_x \cap \RC_x| \epsilon^2} + O(\tfrac{\log n}{k})\right)\cdot k \leq \left(\tfrac{2(\delta+\eta)}{\epsilon^2} + O(\tfrac{\log n}{k})\right) \cdot m \cdot k.$$

	On the other hand, since $q_x$ was found dense in $\eps^2 \cdot m$ partitions, we have the following lower bound on the denominator,
	
		$$\sum_{j \in [m]: q_x \text{ is } j\text{-dense}}  \psi_{\RC_x,j}(q_x) \geq
        \eps^2m\cdot \eps^2k=\eps^4 \cdot m \cdot k.$$
		
		Summing up, we obtain that Eqn. \eqref{eq::prob_fail}
                is at most, for $k=\Omega(\log^2 n)$:
		
		$$	\frac{\left(\tfrac{2(\delta+\eta)}{\epsilon^2} + O(\tfrac{1}{\log n})\right) \cdot m \cdot k}{\eps^4 \cdot m \cdot k}	\leq 2 \cdot \frac{\delta + \eta}{\eps^6} + O(\frac{\eps^{-4}}{\log n}).$$
		
		We conclude that the probability of success can therefore be lower bounded by,
				
$$\Pr_{\chi \sim p}
		\left[v \between_{\kappa_j^{t+1}} \pi[v] \text{ for each
                  } v \in q_x\cap \RC_x \right]
 \geq 1-  2 \cdot \tfrac{\delta + \eta}{\eps^6} - O(\tfrac{\eps^{-4}}{\log n})$$
				
				as needed.
\end{proof}



